An Ontology for Defect Detection in Metal Additive Manufacturing

A key challenge for Industry 4.0 applications is to develop control systems for automated manufacturing services that are capable of addressing both data integration and semantic interoperability issues, as well as monitoring and decision making tasks. To address such an issue in advanced manufacturing systems, principled knowledge representation approaches based on formal ontologies have been proposed as a foundation to information management and maintenance in presence of heterogeneous data sources. In addition, ontologies provide reasoning and querying capabilities to aid domain experts and end users in the context of constraint validation and decision making. Finally, ontology-based approaches to advanced manufacturing services can support the explainability and interpretability of the behaviour of monitoring, control, and simulation systems that are based on black-box machine learning algorithms. In this work, we provide a novel ontology for the classification of process-induced defects known from the metal additive manufacturing literature. Together with a formal representation of the characterising features and sources of defects, we integrate our knowledge base with state-of-the-art ontologies in the field. Our knowledge base aims at enhancing the modelling capabilities of additive manufacturing ontologies by adding further defect analysis terminology and diagnostic inference features.

==> ArXiv/main/sec_conc.tex <==
%
\section{Conclusion}\label{sec:conclusions}
%
\noindent
In the present contribution, we have introduced an OWL 2 ontology to represent MAM defects, together with their constituting features and sources. Our ontology aims at filling a gap in the literature on AM knowledge bases, providing dedicated vocabulary and axioms to capture specific defect-related domain knowledge. To provide additional expressivity and modelling capabilities, we have also integrated our ontology with several upper-level ontologies, as well as domain-specific ontologies from different domains.

As future steps, we plan to extend \emph{DefectOnt} with the capability of relating defects with measured quantities coming from either \textit{in-situ} or \textit{ex-situ} measurements.
Moreover, we are interested in improving the alignment of \DefectOnt with upper ontology or domain-specific knowledge bases from the AM literature.
In a similar direction, to foster the integration of heterogeneous data sources, we plan to consider ontology-based data access techniques and frameworks, focusing in particular on the OWL 2 QL Profile~\cite{KonEtAl13}.
%Ontology-Based Data Access with Databases: A Short Course
Finally, we are interested in investigating the addition of a temporal dimension to our ontology, for temporal data modelling and predictive analysis~\cite{ArtEtAl13,BaaEtAl13,BraEtAl17,KalEtAl19}
%Temporalizing Ontology-Based Data Access
%Temporal Description Logic for Ontology-Based Data Access
%Ontology-Based Data Access with a Horn Fragment of Metric Temporal Logic
%Ontology-based Access to Temporal Data with Ontop: A Framework Proposal

%
Our long term goal is to use these additional representation and reasoning features to mitigate manufacturing defects, by automatically adjusting those process parameters that are found to be related with the corresponding defect sources.
Indeed, our defect ontology is meant to pave the way towards real-time control systems for MAM processes. In fact, combining machine learning mechanisms with knowledge-based representation and high-level reasoning techniques, it can potentially lead to a self-adaptive system able to perform online diagnosis and troubleshooting. 
%
%\todo{\AM{Rephrase paragraph}} If we can classify potential defects, thanks to the above axioms, we are also able to find the defect sources which are related to that specific defect and, in the last instance, to unveil the complex process-structure-properties relationships occurring in MAM. 

==> ArXiv/main/sec_intro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Introduction}\label{sec:intro}

%%% 
%{\color{red}{
%M:
%Al momento i primi tre paragrafi dell'Intro mi sembrano troppo vaghi, perche' volano troppo alto in merito al ruolo del $(1)$ logical reasoning e della $(2)$ XAI nello sviluppo di sistemi per $(3)$ l'Industry 4.0: tre nozioni che, appunto, mi sembrano un po' troppo generiche per stare tutte assieme in questo modo nell'incipit. Forse e' meglio volare bassi all'inizio, dicendo prima le solite cose sulla MAM e le ontologie, e poi gradualmente metterle assieme (anche immaginando scenari a lungo termine), spiegando chiaramente il nostro contributo e come questo si connette al tema dell'integrazione di MAM processes e ontologie.
%
%In questo senso, se sei d'accordo, vorrei ri-organizzare un po' l'Intro come segue.
%\begin{enumerate}
%\item Presentiamo prima la MAM come componente nativa e portante dell'Industry 4.0.
%\item Spieghiamo poi cosa sono le ontologie e come possono essere utilizzate in relazione ai MAM production services per quanto riguarda:
%\begin{itemize}
%\item[$(2.1)$] digitalisation, data management and integration, and semantic interoperability; \item[$(2.2)$] automation, maintenance and decision making support
%\begin{itemize}
%	\item Come prospettiva a lungo termine legata al Punto $(2.2)$, potremmo qui fare cenno alla possibilita' di integrare sistemi di controllo real-time dei production processes basati su algoritmi di apprendimento automatico con ontologie. Questa integrazione ha come obiettivo (nel filone dei sistemi di eXplainable AI) di perfezionare le capacita' diagnostiche dei control systems, sia $(i)$ migliorando, grazie alle reasoning capabilities basate su ontologie, la loro capacita' di riconfigurare in real-time i parametri di stampa in funzione dei difetti individuati, sia $(ii)$ fornendo risposte esplicative alle queries dell'utente circa lo stato di un processo.
%\end{itemize}	
%\end{itemize}
%\item Illustriamo cosa facciamo nel nostro lavoro, che si inserisce nel contesto dei Punti $(2.1)$ e $(2.2)$. Proponiamo una Defect Ontology, integrata in maniera modulare con altre AM ontologies selezionate dalla letteratura, che permette (a differenza dalle ontologie domain-specific sviluppate finora) di:
%\begin{itemize}
%	\item[$(i)$] formalizzare la conoscenza dei domain experts circa difetti principali riscontrabili nei MAM processes;
%	\item[$(ii)$] rispondere a competency questions e queries degli utenti circa la natura, l'origine, e le caratteristiche di difetti riscontrati nel contesto di un processo di stampa
%	\item[$(iii)$] mettere in relazione le proprieta' dei difetti di stampa con ulteriori elementi costitutivi del processo stesso, concettualizzati attraverso le altre AM ontologies prese dalla letteratura.
%\end{itemize}
%\end{enumerate}
%}}


%\todo[inline]{\AM{@AM work on the intro}}
\noindent
Fully automated manufacturing systems,
as well as
%either based on high-volume outputs or on
production-as-a-service frameworks, represent a cornerstone of Industry 4.0 applications~\cite{gaiardelli2021product}.
%https://ieeexplore.ieee.org/document/8398543
%https://www.diag.uniroma1.it/degiacom/papers/2022/aij2022dflps.pdf
In this context, additive manufacturing (AM), and specifically \emph{metal additive manufacturing} (MAM), is
%a technology
particularly suited to
industrial
%Industry 4.0
paradigms based on automation, flexibility, and efficiency.
Indeed, MAM can be considered as a native digital technology, providing a seamless workflow from the digital design environment to the final product, which can be potentially completed without any human intervention~\cite{Gibson2015}.

However, a broader adoption of MAM technologies in industry is still hindered by such factors as:
%https://amfg.ai/2019/10/08/10-of-the-biggest-challenges-in-scaling-additive-manufacturing-for-production-expert-roundup/
\begin{enumerate*}[label=$(\roman*)$]
\item lack of widely adopted standardisations and specifications of material properties, machines, and processes~\cite{king2015laser};
%https://www.rpplusm.com/blog/posts/material-database-complete/
	\item lack of adequate digital infrastructures, and interoperability issues between different production environments~\cite{badiru2017additive};
	\item lack of
accessible interfaces
providing
%queryable and explainable
process information that is easily interpretable by non-experts~\cite{lawrence2017advances};
%https://amfg.ai/2019/03/15/quality-assurance-for-metal-3d-printing-solving-3-common-challenges/
%https://www.sciencedirect.com/science/article/pii/S2214860421000890
	\item lack of advanced control systems capable of automatically adjusting, at run-time, the production parameters~\cite{mani2015};
	\item challenges in quality assurance due part accuracy and variability~\cite{leary2019design}.
\end{enumerate*}

Thus, achieving semantically transparent and interoperable data sets and systems, to address Points~$(i)$, $(ii)$ and $(iii)$ above, is  arguably
of paramount importance.
%crucial
%to fully exploit the design flexibility for scalable production services originally promised by the MAM technology~\cite{bian2017laser}, hence contributing to its wider adoption in industrial settings.
%}}
%
In this direction, several approaches based on ontology engineering and knowledge representation techniques have been proposed~\cite{garetti2012role,belkadi2016towards,SanEtAl19,preisig2020ontologies}
%A Description Logic Based Ontology for Knowledge Representation in Process Planning for Laser Powder Bed Fusion
%Ontology-based knowledge representation for additive manufacturing
%
Broadly conceived as formal specifications of conceptualisations over a domain of interest, computational ontologies (cf.~\cite{GuaEtAl09} and references therein) have been in particular investigated as a tool to improve interoperability of additive manufacturing systems that involve human-intensive and domain-expert knowledge management tasks (cf.~Section~\ref{sec:state-of-the-art} for a literature survey).
%Role of ontologies in open automation of manufacturing systems
%
%A Product Life Cycle Ontology for Additive Manufacturing
%A Design for Additive Manufacturing Ontology
%A Design for Additive Manufacturing Ontology to Support Manufacturability Analysis
%Ontology-based Process Map for Metal Additive Manufacturing
%%As such, they represent valuable tools for information management tasks in knowledge-sensitive contexts, such as the medical or the industrial domains, where structured knowledge from domain experts needs first to be elicited and correctly formalised before being processed and shared in applications.
%For this reason, several domain-specific additive manufacturing ontologies have been proposed.

To the best of our knowledge, however, despite the number of domain-specific ontologies proposed in the literature to address interoperability issues, less attention has been devoted to another crucial aspect of AM applications, in particular of \emph{Powder Bed Fusion} (PBF) MAM: that of \emph{defect diagnosis} and \emph{correction}.
%
PBF is a layer-by-layer process, where a layer of metal powder is spread by means of a roller on top of a build plate, and metal powder particles are selectively melted by means of a localised moving laser heat source \cite{frazier2014metal}.
%
At industrial level, PBF MAM is a widespread technology, due to its capability to deliver parts with high surface quality and remarkable mechanical properties.
%
Nonetheless, the localised nature of the
%resulting 
melt pool induces rapid melting-solidification cycles that are responsible for part deflections and residual stresses \cite{Bartlett2019}. 
%
Moreover, due to their multi-scale and multi-physics nature,
%physical 
phenomena involved in PBF processes are difficult to control.
%
Finally, the overall process is characterised by complex and not yet fully understood relationships among material microstructure, part geometry, process parameters, and mechanical properties and performances \cite{smith2016linking}.
%
Such issues can lead to process-induced material discontinuities, e.g. lack-of-fusion and keyhole porosity, balling, crack and delamination \cite{DUPLESSIS2020108385}.

Even if these process-related defects play a key role influencing part properties and performances (e.g., elastic and elastoplastic behaviour, ultimate tensile stress, and fatigue life), an ontology-based representation of MAM defects, together with their main properties surveyed in the literature~\cite{bian2017laser}, is not yet available.
Such a principled approach, integrating observational data with formalised domain knowledge to determine the causality links and the complex process-structure-property relationships in manufacturing processes, represents an important preliminary step for the development of reliable monitoring and control systems capable of addressing Points~$(iv)$ and~$(v)$ above~\cite{debroy2018additive}.
%Even if process-related defects play a key role influencing part properties and performances (e.g., elastic and elastoplastic behaviour, ultimate tensile stress, and fatigue life), a rigorous knowledge-based representation of MAM defects is not yet available.
 %
%In order to develop reliable monitoring or control systems capable of addressing Points~$(iv)$ and~$(v)$ above, a rigorous representation of production defects known to affect MAM processes, together with a formalisation of their main properties surveyed in the literature~\cite{?}, is of primary importance.
%
%
%A principled approach integrating observational data with domain knowledge to determine the causality links and the complex process-structure-property relationships in manufacturing processes
%represents, thus, an important open problem
%%is thus one of the main issues
%in AM research~\cite{debroy2018additive}. 
%control systems with automated defect diagnosis and correction capabilities is an where structured knowledge from domain experts be elicited and correctly formalised before being processed and shared in applications


Our contribution aims at filling this gap, by introducing the novel \DefectOnt \footnote{\href{https://github.com/AndreaMazzullo/DefectOnt}{\texttt{https://github.com/AndreaMazzullo/DefectOnt}.}} ontology for MAM, specifically PBF-based, defects.
%
This ontology relies on a modular structure, and it aligns with other upper and domain-specific ontologies from the literature, to favour development, interoperability and maintenance.
It includes axioms covering the following dimensions:
\begin{enumerate*}[label=$(\roman*)$]
\item MAM-based categories of defects and related properties;
\item spatial notions to express geometrical and topological characteristics;
\item dimensional characteristics requiring a vocabulary of metrological terms;
\item sensor-related concepts for observational properties.
\end{enumerate*}
\DefectOnt is implemented in the OWL 2~\cite{GraEtAl08}\footnote{\href{https://www.w3.org/TR/owl2-overview/}{\texttt{https://www.w3.org/TR/owl2-overview/}.}}, using the open-source Prot\'{e}g\'{e} ontology editor~\cite{KnuEtAl04}\footnote{\href{https://protege.stanford.edu/}{\texttt{https://protege.stanford.edu/}.}}.
%
%The \DefectOnt ontology contributes to the following aspects:
%first, it provides to domain experts a structured framework for the classification and analysis of MAM defects; secondly, it 

%\todo[inline]{\AM{working here, todo add our contribution}}


The present article is organised as follow. In Section~\ref{sec:state-of-the-art}, we discuss related work on MAM defects and AM ontologies. Then, in Section~\ref{sec:ont-design-meth}, the design methodology and the development phases of our MAM defect ontology are described. In Section~\ref{sec:AM-defect-ontology},  we illustrate the \emph{DefectOnt} ontology, presenting in detail the modules that constitute it. Finally, in Section~\ref{sec:conclusions}, we discuss future research directions and the main conclusions of the present work.


%{\color{red}{
%Modern industrial systems go towards fully digitalized and automatized factories which are one the cornerstone of Industry 4.0. To achieve such an ambitious goal, it is essential to introduce an additional layer of logical reasoning to the state-of-the-art automatic assembly and manufacturing systems, such that these machines can autonomously take actions through a logical-based decision process. 
%
%Explainable Artificial Intelligence (XAI) seems to be an effective approach to provide artificial intelligent systems with more flexible and understandable control algorithms. Due to its ability to take explainable decisions based on the input data or user queries, XAI can address the contemporary challenges of Industry 4.0 \cite{bhatt2020expanding,mehta2019high}. In fact, adding a further layer of reasoning through modern computational ontologies to traditional machine learning approaches can foster the industry to complete its step towards a fully digitalized system \cite{liang2018ontology}.    
%In particular, Metal Additive Manufacturing (MAM) seems to be the manufacturing technology more suitable to be integrated within Industry 4.0 paradigms. In fact, MAM can be considered as a native digital technology since it provides a seamless workflow from the digital design environment to the final product which can be potentially completed without any human intervention \cite{Gibson2015}. However, a broader adoption of MAM technologies in industry is still hindered by the lack of standardization and reproducibility of such a technology. Therefore, the possibility to achieve a real-time monitoring and control system is nowadays crucial to fully exploit possibility of an almost unlimited designed freedom in large-scale manufacturing originally promised by MAM technology \cite{bian2017laser}.
%
%In the present work, we introduce an OWL ontology module to represent the knowledge about MAM defects and their source. Such a module is intended to be a standalone set of logical entities that can easily merged with any available AM ontology. However, it is only when merged with broader AM ontologies that it can be effectively used to generate a knowledge-based representation of the MAM process that can be employed, for instance, for XAI-based real-time control systems. Therefore, in this work we also present the merging of the proposed module into a state-of-the-art AM ontology.
%
%The present contribution is organized as follow. In \ref{sec:state-of-the-art}, the state-of-the-art of manufacturing ontology and, in particular, of additive manufacturing ontologies is presented. \ref{sec:AM-defect-module} the MAM defects ontology module is described in detail. In \ref{ssec:AMmodule}, the axioms necessary to merge the presented module within an AM ontology from the literature are discussed together with the prospective application of such an extended ontology. Finally, in \ref{sec:conslusions}, e draw the main conclusion and further outlook of the present work.
%}}

==> ArXiv/main/sec_ontodesign.tex <==
\section{Ontology design and development}
\label{sec:ont-design-meth}
\noindent
To develop our ontology, we followed the approach proposed by~\citet{RamEtAl20}, with the adoption of the NeOn Methodology~\cite{SuaEtAl12} and in particular of the Six-Phase + Merging Phase Waterfall Ontology Network Life Cycle Model.
This model, allowing for a flexible interplay between pre-existing ontological and non-ontological resources, consists of the following phases, which will be detailed in the remainder of this section:
%$(i)$
initiation,
%$(ii)$
reuse,
%$(iii)$
merging,
%$(iv)$
re-engineering,
%$(v)$
design,
%$(vi)$
implementation,
and
%$(vii)$
maintenance.

\subsection{Initiation phase}
%\paragraph{{\bf Initiation phase}}
\noindent
As by the methodological framework of~\citet{SuaEtAl09},
%HowtoWriteandUsetheOntologyRequirementsSpecificationDocument
we initially developed an Ontology Requirements Specification Document (ORSD), summarised in Table~\ref{tab:orsd}, with the following goals:
defining the purpose and the scope of our ontology; selecting the implementation languages; identifying intended users and uses of the ontology; formulating in natural language groups of competency questions (CQs), to be expressed and answered by our ontology;
providing a pre-glossary of terms appearing in the CQs.
%


To better illustrate the purpose and the intended uses of our ontology, we present the following simplified scenario, involving a MAM production service monitored and regulated by a control system relying, for instance, on a machine learning architecture.
Suppose that, during a 3D printing process, the monitoring system detects a feature that is classified (by means of, e.g., a pre-trained convolutional neural network) as a porosity defect, consisting of a void encapsulated within bulk material.
Moreover, assume that the system controller (based on, e.g., a reinforcement learning mechanism), in an attempt to mitigate the propagation of the feature, sequentially modifies relevant build chamber parameters, powder handling and deposition system parameters, and the laser scanning speed, observing that only the latter has an impact on limiting the defect.
The purpose of our ontology is to formalise the domain knowledge required to infer that the detected porosity is an instance of a process-induced defect, rather than of an equipment-induced one (given that all other possible equipment-related parameters have been ruled out as influences on the feature).

In such contexts, our ontology can be used to:
%$(i)$
provide a (both machine- and human-readable) structured representation of MAM defects, including their main characteristics and mutual relationships;
%$(ii)$
enrich the online monitoring and troubleshooting capabilities of controllers by means of logic-based reasoning services;
%$(iii)$
improve the user interface to MAM production processes, integrating black-box controller systems with a user-queryable and explainable diagnostic framework.

Finally, we have grouped the CQs along four dimensions, constituting the backbone of our ontology modular structure:
\begin{enumerate*}[label=$(\roman*)$]
\item MAM-related (CQAm);
\item spatial-related (CQSp);
\item measure-related (CQMe);
and
\item sensor-related (CQSe).
\end{enumerate*}

%\setlist[itemize]{topsep=0pt,before=\leavevmode\vspace{-1.5em}}
\setlist[description]{font=\normalfont\itshape}
%style=nextline

\begin{table}
\centering
\caption{Summary of \emph{DefectOnt} Ontology Requirements Specification Document.}
\label{tab:orsd}
\begin{tabular}{ p{\textwidth} }
 \hline
%
{\footnotesize{
\begin{description}
%[style=nextline]
%[noitemsep,topsep=0pt]
	%
	\item[{Purpose}] Representation of and reasoning about defects and defect sources in MAM processes, enhancing inference-based diagnostic capabilities to support the user in production control and decision making phases.
	%
	\item[{Scope}]
	Diagnosis and troubleshooting in MAM machines and processes. Potential application contexts are research laboratories and industrial settings.
	%
	\item[{Implementation languages}] 
	OWL 2 (description logic syntax).
	%
	\item[{Intended users}]
	Domain experts, product designers, company employees.
	%
	\item[{Intended uses}]
	\begin{itemize}	[topsep=0pt,before=\leavevmode\vspace{-1.5em}]
		\item[]
		\item Aid user understanding of the classification of MAM defects and corresponding sources.
		\item Enhance automated MAM process control systems with high-level reasoning capabilities.
		\item Guide user interaction with automated MAM process control systems by means of ontology-based explainable diagnostic services.
	\end{itemize}
	%
	\item[{Ontology requirements}]
		\begin{itemize}[topsep=0pt,before=\leavevmode\vspace{-1.5em}]
			%
			\item[]
			%
			\item Non-functional requirements:
%			Allow for inference-based defect diagnosis to support the user in MAM production control and decision making phases.
			Ontology based on defect classifications from state-of-the-art surveys in the MAM literature.
%			(cf.~\cite{?} and references therein).
			%
			\item Functional requirements: Groups of competency questions (CQs).
%			\todo[inline]{Both: These CQs have to be modified and to appear in the text.}
			\begin{itemize}
				%
				\item[CQAm] MAM-related CQs
				\begin{enumerate}[label=CQAm.\arabic*]
%					\item[CQAm.1] Is the feature ${\sf d}$ an instance of a defect?
					\item Is the feature ${\sf d}$ an instance of a porosity defect?
%					\item[CQAm.3] Which type of defect is defect ${\sf d}$?
%					\item[CQAm.4] By which parameters can defect ${\sf d}$ be influenced?
					\item Is defect ${\sf d}$ induced by a process parameter?
					\item \ldots
				\end{enumerate}
				\item[CQSp] Spatial-related CQs
				\begin{enumerate}[label=CQSp.\arabic*]
					\item Is the MAM product {\sf pr} affected by any equipment-induced surface defects?
					\item Are there balling defects located on the surface layers of product {\sf pr}?
					\item \ldots
%					\item[CQSp.1] Is there an instance of a balling defect overlapping with a surface layer?
%					\item[CQSp.2] What is the length in metres of the cracking defect instance {\sf d}?
%					\item[CQSp.3] \ldots
%%					\item[CQSp.3] What is the volume of the bounding box {\sf b} for balling defect {\sf d}?
%%					\item[CQSp.3] What is the dimension of {\sf d}?
%%					\item[CQSp.1] Where is located the defect in the component?
%%					\item[CQSp.2] What is the morphology of the defect?
%%					\item[CQSp.3] What is the size of the defect?
				\end{enumerate}
				%
				\item[CQMe] Measure-related CQs
					\begin{enumerate}[label=CQMe.\arabic*]
						\item What is the melt pool temperature in degrees Celsius?
	\item What is the thickness in millimetres of layer {\sf l}?
	\item What is the length in metres of the cracking defect instance {\sf d}?
	\item \ldots
%					\item[CQMe.1] Which quantities can be measured by the XXX sensor?
%					\item[CQMe.2] Which quantities can be measured by the YYY sensor?
%					\item[CQMe.3] Which quantities can be measured by the ZZZ sensor?
%					\item[CQMe.4] What unit of measurement is used by the XXX sensor?
%					\item[CQMe.5] What unit of measurement is used by the YYY sensor?
%					\item[CQMe.6] What unit of measurement is used by the ZZZ sensor?
					\end{enumerate}
				\item[CQSe] Sensor-related CQs
				\begin{enumerate}
					\item[CQSe.1] Which sensors are hosted by platform {\sf pl}?
					\item[CQSe.2] Does any sensor hosted by platform {\sf pl} observe an instance of a porosity defect?
						\item[CQSe.3] \ldots
%					Is the feature of interest of observation {\sf o} made by sensor {\sf s} an instance of a porosity defect?
%					\item[CQSe.1] Which sensors are installed in the machine?
%					\item[CQSe.2] Which feature of interests can be measured?
				\end{enumerate}
				%
			\end{itemize}
		\end{itemize}
	\item[Pre-glossary of terms] Defect, porosity, cracking, balling, equipment-induced defect, process-induced defect, product, layer, sensor, platform, melt pool, \ldots
\end{description}
}}\\
\hline
%
\end{tabular}
\end{table}


\subsection{Reuse phase}
\noindent
%\paragraph{{\bf Reuse Phase}}
%
In order to obtain the domain knowledge required to express and formalise relevant properties of MAM defects, we collect material from both ontological and non-ontological resources. While the latter are based on (not yet formalised) literature on MAM defects, we relied on already existing additive manufacturing ontologies to gather structured knowledge related to MAM processes.
The selected ontologies were preferred over other available resources based on the following criteria:
(i) possibility of integrating class and property hierarchies with other non-ontological resources; and (ii) vocabularies capable of expressing properties of defects determined by the CQs.
In the following, we present the relevant material divided along the four dimensions determined by the groups of CQs.


\begin{description}[font=\normalfont\itshape]
	\item[MAM-related resources]
%	\todo[inline]{\AM{todo add}}
	As our main non-ontological resources related to MAM defects, we identify:~\citet{grasso2017process}, providing a classification that relates each kind of defect with the main causes analysed in the literature;
	\citet{malekipour2018common}, similar to the previous article in scope and purpose, but providing a different taxonomy of defects;
	\citet{snow2020invited}, focusing mainly on the internal porosity classification.
	To exploit formal representations of the main notions involved in the MAM domain, while maintaining a neutral and interoperable environment, we use instead the following ontologies:
	NIST AM~\cite{WitEtAl16}\footnote{\href{https://github.com/iassouroko/AMontology}{\texttt{https://github.com/iassouroko/AMontology}.}};
	and
	Onto4additive~\cite{SanEtAl19}\footnote{\href{https://ontohub.org/repositories/additive-manufacturing}{\texttt{https://ontohub.org/repositories/additive-manufacturing}.}}.
			Finally, as a methodological guidance and as a source for specific module development (cf.~\emph{Measure-related resources}),
%			~\ref{item:measureresource}
			we rely on the \emph{ExtruOnt} ontology~\cite{RamEtAl20}\footnote{\href{http://siul02.si.ehu.es/bdi/ontologies/ExtruOnt/docs/}{\texttt{http://siul02.si.ehu.es/bdi/ontologies/ExtruOnt/docs/}.}}.

	
	\item[Spatial-related resources] 
%	\todo[inline]{\AM{todo add}}
	To model spatial-related, geometrical or topological, concepts and relations, we choose GeoSPARQL 1.1~\cite{CarEtAl22}\footnote{\href{https://opengeospatial.github.io/ogc-geosparql/geosparql11/index.html}{\texttt{https://opengeospatial.github.io/ogc-geosparql/geosparql11/index.html}.}}. Additional spatial-related concepts are inherited from the MASON~\cite{LemEtAl06}\footnote{\href{https://sourceforge.net/projects/mason-onto/}{\texttt{https://sourceforge.net/projects/mason-onto/}.}} ontology.
%	M. Perry and J. Herring, OGC GeoSPARQL - A geographic query language for RDF data
%	GeoSPARQL 1.1: Motivations, Details and Applications of the Decadal Update to the Most Important Geospatial LOD Standard


	\item[Measure-related resources]\label{item:measureresource} To express metrological features in our ontology, we rely directly on the \emph{OM4ExtruOnt} module developed by~\citet{RamEtAl20}. This module is obtained by removing all the classes and properties not relevant to the manufacturing setting from the OM ontology~\cite{RijEtAl13}\footnote{\href{https://github.com/HajoRijgersberg/OM}{\texttt{https://github.com/HajoRijgersberg/OM}.}}.
	
	
	\item[Sensor-related resources]
	As main ontological resource to conceptualise observation- and sensor-related notions, we select the Semantic Sensor Network (SSN) ontology~\cite{HalEtAl19}\footnote{\href{https://www.w3.org/TR/vocab-ssn/}{\texttt{https://www.w3.org/TR/vocab-ssn/}.}}. 
%	A. Haller, K. Janowicz, S.J.D. Cox, M. Lefrançois, K. Tay- 16 lor, D.L. Phuoc, J. Lieberman, R. García-Castro, R. Atkinson 17 and C. Stadler, The modular SSN ontology: A joint W3C and 18 OGC standard specifying the semantics of sensors, observations, sampling, and actuation
	
\end{description}

\subsection{Merging phase}
\noindent
%\paragraph{{\bf Merging Phase}}
%
With the aim of improving semantic interoperability and knowledge exchange in applications, we structure the upper or domain ontologies identified in the reuse phase so to be aligned with the \DefectOnt framework.
In order to merge these ontologies, we perform the following steps.
\begin{enumerate}[label=$(\roman*)$]
	\item We select higher-level classes (with respect to our defect-related concepts) to be introduced in the \DefectOnt hierarchy (e.g., {\sf Entity} from MASON ontology,  {\sf Abstract}, {\sf Physical}, {\sf Characteristic} from NIST AM ontology, {\sf PhysicalObject} from Onto4Additive ontology, {\sf SpatialObject} from GeoSPARQL ontology, {\sf Property} from SSN ontology).
	\item We identify classes that (for our modelling purposes) formalise interchangeable notions, in order to set them as equivalent in the class hierarchy of the \DefectOnt ontology (e.g., {\sf PhysicalObject} from the Onto4Additive and {\sf SpatialObject} from the GeoSPARQL; {\sf Characteristic} from NIST and {\sf Property} from SSN).
	\item We devise class sub-hierarchies to connect the vocabulary and the axioms from different ontologies (e.g. {\sf Characteristic} from NIST and {\sf ObservableCharacteristic} from SSN introduced as subclass; {\sf Physical} from NIST and {\sf SpatialObject} from GeoSPARQL introduced as subclass).
\end{enumerate}



\subsection{Re-engineering phase}
\noindent
%\paragraph{{\bf Re-engineering Phase}}
As already mentioned, our main non-ontological resources identified in the reuse phase are~\citet{grasso2017process} (in particular, Table~1 and references therein), \citet{snow2020invited}, and \citet{malekipour2018common}.
%As our main non-ontological resources, we focus on~\citet{grasso2017process}, and in particular on their Table~1 (and references therein), \citet{snow2020invited} that focuses mainly on the internal porosity classification, and \citet{malekipour2018common}. 
These references are used to extract a conceptual framework based on defect types and corresponding sources, compatible with the purpose, the intended uses, and the implementation languages of the \DefectOnt ontology.




\subsection{Design phase}
%\paragraph{{\bf Design Phase}}
\noindent
To facilitate development, interoperability, and maintenance (in line with the approach by~\citet{RamEtAl20}), our \emph{DefectOnt} ontology is based on a modular structure, reflecting the dimensions that emerge with the ORSD development in the initiation phase.
%%
The \DefectOnt ontology consists of the following three modules.
\begin{enumerate}[label={\arabic*.}]
	\item \emph{MAM4DefectOnt}, a MAM-related module importing the following ontologies:
			\begin{enumerate}[label*=\arabic*]
			\item \emph{NIST4DefectOnt}, a module obtained from the NIST AM ontology;
			\item \emph{ONTO4ADD4DefectOnt}, derived from the \emph{Onto4Additive} ontology;
			\item \emph{Spatial4DefectOnt}, to represent spatial-related notions, in turn consisting of the following modules:
			\begin{enumerate}[label*=.\arabic*]
				\item \emph{GeoSPARQL4DefectOnt}, obtained from the GeoSPARQL1.1 ontology;
				\item \emph{MASON4DefectOnt}, derived from the MASON ontology.
			\end{enumerate}
		\end{enumerate}
	\item \emph{Measure4DefectOnt}, a measuring-related module importing \emph{OM4ExtruOnt}, a submodule originally developed for the \emph{ExtruOnt} ontology from the OM ontology.
	\item \emph{Sensor4DefectOnt}, a sensor-related module consisting of the submodule \emph{SSN4DefectOnt} obtained from the SSN ontology.
\end{enumerate}
%The four modules that constitutes the ontology, and that will be detailed in Section~\ref{sec:AM-defect-ontology} below, are the following (cf. Figure~\ref{fig:mainclasses}):
%$(1)$ the MAM module \emph{MAM4DefectOnt}, defining properties of defects that involve MAM-related notions;
%$(2)$ the spatial module \emph{Spatial4DefectOnt}, for the topological and geometrical characteristics of defects
%$(3)$ the measure module \emph{Measure4DefectOnt}, allowing to refer to metrological properties of defects;
%and
%$(4)$ the sensor module \emph{Sensor4DefectOnt}, introducing the terminology required for observable properties and sensor platforms.
%In turn, these modules require the following submodules:
%$(1)$
%%\emph{MAM4DefectOnt} module relies on three submodules 
%\emph{MASON4DefectOnt}, \emph{ONTO4ADD4DefectOnt}, and \emph{NIST4DefectOnt};
%%the module \emph{Spatial4DefectOnt} on two
%$(2)$ \emph{GeoSPARQL4DefectOnt} and \emph{MASON4DefectOnt};
%%while the \emph{Measure4DefectOnt} and \emph{Sensor4DefectOnt} modules contain one submodule each
%$(3)$ \emph{OM4ExtruOnt4DefectOnt};
%and
%$(4)$ \emph{SSN4DefectOnt}.
%%respectively).

To design our ontology modules, we perform the following main steps:

\begin{enumerate}[label=$(\roman*)$]
%
	\item\label{item:one} In a preliminary class hierarchy of the \emph{MAM4DefectOnt} module, we structure the domain knowledge formalised from the non-ontological resources during the re-engineering phase (e.g., by introducing the {\sf Defect} class and related sub-classes).
%
	\item\label{item:two} We prune the class hierarchies of the ontologies selected in the re-use phase, maintaining only the most relevant vocabulary and axioms,
%		to the \DefectOnt purposes,
		to obtain the submodules for \emph{MAM4DefectOnt}, as well as for its submodule \emph{Spatial4DefectOnt}, \emph{Measure4DefectOnt}, and \emph{Sensor4DefectOnt}.
%
	\item\label{item:three} We refine the ontology formalisation of Step~\ref{item:one} by adding to the \emph{MAM4DefectOnt} module axioms based on classes and properties from submodules devised in Step~\ref{item:two} (e.g., {\sf Defect}-related axioms based on the {\sf influencedBy} property from NIST ontology).
%
	\item We enrich the class hierarchies of Step~\ref{item:two} submodules to further improve the ontology formalisation process (e.g., introducing in \emph{Spatial4DefectOnto} the class {\sf Ball} as subclass of {\sf Geometric\_entity} from MASON ontology).
%
	\item We modify class hierarchies and axioms from the submodules obtained in Step~\ref{item:two} to adhere to the non-ontological resource formalisation performed in Steps~\ref{item:one} and~\ref{item:three} (e.g., by setting {\sf EquipmentParameter} as a sibling class of {\sf ProcessParameter}, rather than subclass (as in NIST), in accordance with~\citet{grasso2017process}).
%
	\item We perform a terminological normalisation process, to align the naming scheme for short IRIs of \DefectOnt classes (e.g., by changing {\sf influencedBy} from NIST to {\sf isInfluencedBy}; {\sf Geometry\_entity} from MASON to {\sf GeometricEntity}).
\end{enumerate}





\subsection{Implementation phase}
%\paragraph{{\bf Implementation Phase}}
\noindent
Initially partly expressed by means of a description logic (DL) language~\cite{BaaEtAl17}, our ontology is fully implemented in OWL 2, using the Prot\'{e}g\'{e} ontology editor.
According to the Prot\'{e}g\'{e} ontology metrics, \DefectOnt can be expressed with the logical constructs provided by the $\mathcal{ALCHOIQ}(\mathcal{D})$ DL language.




\subsection{Maintenance phase}
%\paragraph{{\bf Maintenance Phase}}
%
\noindent
As a time-consuming and error-prone task, the knowledge extraction process for the design of the \DefectOnt ontology comes with a (still active) maintenance protocol. As prescribed by the selected Ontology Network Life Cycle Model, whenever a modelling error is detected, our ontology re-enters one among the reuse, merging, re-engineering, or design phases for corrections.



==> ArXiv/main/sec_ontomodule.tex <==
\section{Ontology modules}
\label{sec:AM-defect-ontology}

\noindent
%As mentioned in Section~\ref{sec:ont-design-meth}, the \DefectOnt ontology consists of the following three modules.
%\begin{enumerate}[label={\arabic*.}]
%	\item \emph{MAM4DefectOnt}, a MAM-related module importing the following ontologies:
%			\begin{enumerate}[label*=\arabic*]
%			\item \emph{NIST4DefectOnt}, a module obtained from the NIST AM ontology;
%			\item \emph{ONTO4ADD4DefectOnt}, derived from the \emph{Onto4Additive} ontology;
%			\item \emph{Spatial4DefectOnt}, to represent spatial-related notions, in turn consisting of the following modules:
%			\begin{enumerate}[label*=.\arabic*]
%				\item \emph{GeoSPARQL4DefectOnt}, obtained from the GeoSPARQL1.1 ontology;
%				\item \emph{MASON4DefectOnt}, derived from the MASON ontology.
%			\end{enumerate}
%		\end{enumerate}
%	\item \emph{Measure4DefectOnt}, a measuring-related module importing \emph{OM4ExtruOnt4DefectOnt}, a submodule originally developed for the \emph{ExtruOnt} ontology from the OM ontology.
%	\item \emph{Sensor4DefectOnt}, a sensor-related module consisting of the submodule \emph{SSN4DefectOnt} obtained from the SSN ontology.
%\end{enumerate}
%%$(1)$ the MAM module \emph{MAM4DefectOnt};
%%$(2)$ the spatial module \emph{Spatial4DefectOnt};
%%$(3)$ the measure module \emph{Measure4DefectOnt};
%%and $(4)$ the sensor module \emph{Sensor4DefectOnt}.
%%In turn, these modules contain the following submodules:
%%\begin{enumerate}[label=$(\arabic*')$]
%%\item
%%%\emph{DefectCore4DefectOnt},
%%\emph{NIST4DefectOnt},  \emph{ONTO4ADD4DefectOnt},
%%\emph{Spatial4DefectOnt}
%%%\emph{MASON4DefectOnt},
%%\item \emph{OM4ExtruOnt4DefectOnt};
%%\item \emph{SSN4DefectOnt}.
%%\end{enumerate}
%%Finally, the \emph{Spatial4DefectOnt} consists of the following modules: \emph{GeoSPARQL4DefectOnt}, obtained from the GeoSPARQL1.1 ontology; \emph{MASON4DefectOnt}, derived from the MASON ontology.
Along the dimensions identified in the ontology development process (cf. Section~\ref{sec:ont-design-meth}) and depicted in Figure~\ref{fig:mainclasses}, the \DefectOnt modules provide relevant vocabulary and formalise the domain knowledge required to represent the main features of production defects possibly occurring in MAM processes.
We illustrate them in detail in the rest of this section, using DL syntax~\cite{BaaEtAl17} for the OWL 2 axioms here presented.
%where we propose a knowledge-based representation of the main defects occurring during MAM processes and their corresponding sources.
%As depicted in \ref{fig:mainclasses} the ontology is composed by two main classes: \texttt{Defect} and \texttt{DefectSource}, such that each element of \texttt{Defect} requires to have a source.










\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5},
%	every label/.append style={align=center},
    >=stealth,
    box/.style = {text width=2cm, font=\small},
    node distance=3cm,
    database/.style={
      cylinder,
%      cylinder uses custom fill,
%      cylinder body fill=green!20,
%      cylinder end fill=green!20,
      shape border rotate=90,
      aspect=0.25,
      draw
    }
  ]
    \node[database] (defectont) at (0,0) {\shortstack{\DefectOnt\\Ontology}};
    
    
    % MAM module
    \node[database] (mam) at (0,-3) {\shortstack{\emph{MAM}\\\emph{4DefectOnt}}};
    %
    
        \node[database, align=center] (nist) at (-4.5,-4.5)
        {
        \emph{NIST} \\ \emph{4DefectOnt}
        };
%
		\node[database, align=center] (onto4add) at (4.5,-4.5) 
		{
		\emph{ONTO4ADD} \\ \emph{4DefectOnt}
		};   
		 
  % Spatial module
    \node[database] (spatial) at (0,-6) {\shortstack{\emph{Spatial}\\\emph{4DefectOnt}}};
    %
        \node[database, align=center] (geosparql) at (-4,-8) {\emph{GeoSPARQL} \\ \emph{4DefectOnt}};
        \node[database, align=center] (mason2) at (4,-8) {\emph{MASON} \\ \emph{4DefectOnt}};
%    \node[rectangle, rounded corners, draw] (geosparql) at (-2,6) {\shortstack{\emph{GeoSPARQL} \\ \emph{4DefectOnt}}};
%        \node[rectangle, rounded corners, draw] (mason2) at (2,6) {\shortstack{\emph{MASON} \\ \emph{4DefectOnt}}};
    %
    \draw[->] (spatial) -- (geosparql);
    \draw[->] (spatial) -- (mason2);
    
    
    \draw[->] (defectont) -- (mam);
    \draw[->] (mam) -- (nist);
    \draw[->] (mam) -- (spatial);
    \draw[->] (mam) -- (onto4add);
    
% Measure module
    \node[database, align=center] (measure) at (-3,3) {\emph{Measure}\\\emph{4DefectOnt}};
    %
        \node[database, align=center] (om) at (-6,6) {\emph{OM} \\ \emph{4ExtruOnt}};
    %
    \draw[->] (defectont) -- (measure);
    \draw[->] (measure) -- (om);



% Sensor module
    \node[database, align=center] (sensor) at (3,3) {\emph{Sensor}\\\emph{4DefectOnt}};
    %
    \node[database, align=center] (ssn) at (6,6) {\emph{SSN} \\ \emph{4DefectOnt}};
    %
    \draw[->] (defectont) -- (sensor);
    \draw[->] (sensor) -- (ssn);



  \end{tikzpicture}
	\caption{Diagram of the direct import structure for \emph{DefectOnt} modules.}
%	with the corresponding signatures.
%	\todo[inline]{\AM{Figures to discuss/fix}}}
	\label{fig:mainclasses}	
\end{figure}








%\begin{figure}
%\centering
%\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5},
%%	every label/.append style={align=center},
%    >=stealth,
%    box/.style = {text width=2cm, font=\small},
%    node distance=3cm,
%    database/.style={
%      cylinder,
%%      cylinder uses custom fill,
%%      cylinder body fill=green!20,
%%      cylinder end fill=green!20,
%      shape border rotate=90,
%      aspect=0.25,
%      draw
%    }
%  ]
%    \node[database] (defectont) at (0,0) {\shortstack{\DefectOnt\\Ontology}};
%    
%    
%    % MAM module
%    \node[database] (mam) at (-4,0) {\shortstack{\emph{MAM}\\\emph{4DefectOnt}}};
%    %
%    
%        \node[database, align=center] (nist) at (-8,-4)
%        {
%        \emph{NIST} \\ \emph{4DefectOnt}
%        };
%%
%		\node[database, align=center] (onto4add) at (-8,4) 
%		{
%		\emph{ONTO4ADD} \\ \emph{4DefectOnt}
%		};   
%		 
%  % Spatial module
%    \node[database] (spatial) at (-8,0) {\shortstack{\emph{Spatial}\\\emph{4DefectOnt}}};
%    %
%        \node[database, align=center] (geosparql) at (-12,2) {\emph{GeoSPARQL} \\ \emph{4DefectOnt}};
%        \node[database, align=center] (mason2) at (-12,-2) {\emph{MASON} \\ \emph{4DefectOnt}};
%%    \node[rectangle, rounded corners, draw] (geosparql) at (-2,6) {\shortstack{\emph{GeoSPARQL} \\ \emph{4DefectOnt}}};
%%        \node[rectangle, rounded corners, draw] (mason2) at (2,6) {\shortstack{\emph{MASON} \\ \emph{4DefectOnt}}};
%    %
%    \draw[->] (spatial) -- (geosparql);
%    \draw[->] (spatial) -- (mason2);
%    
%    
%    \draw[->] (defectont) -- (mam);
%    \draw[->] (mam) -- (nist);
%    \draw[->] (mam) -- (spatial);
%    \draw[->] (mam) -- (onto4add);
%    
%% Measure module
%    \node[database, align=center] (measure) at (4,4) {\emph{Measure}\\\emph{4DefectOnt}};
%    %
%        \node[database, align=center] (om) at (8,4) {\emph{OM4ExtruOnt} \\ \emph{4DefectOnt}};
%    %
%    \draw[->] (defectont) -- (measure);
%    \draw[->] (measure) -- (om);
%
%
%
%% Sensor module
%    \node[database, align=center] (sensor) at (4,-4) {\emph{Sensor}\\\emph{4DefectOnt}};
%    %
%    \node[database, align=center] (ssn) at (8,-4) {\emph{SSN} \\ \emph{4DefectOnt}};
%    %
%    \draw[->] (defectont) -- (sensor);
%    \draw[->] (sensor) -- (ssn);
%
%
%
%  \end{tikzpicture}
%	\caption{Diagram of the direct import structure for \emph{DefectOnt} modules.}
%%	with the corresponding signatures.
%%	\todo[inline]{\AM{Figures to discuss/fix}}}
%	\label{fig:mainclasses}	
%\end{figure}










%\begin{figure}
%\centering
%\begin{tikzpicture}[scale=0.5, every node/.style={scale=0.5},
%%	every label/.append style={align=center},
%    >=stealth,
%    box/.style = {text width=2cm, font=\small},
%    node distance=3cm,
%    database/.style={
%      cylinder,
%%      cylinder uses custom fill,
%%      cylinder body fill=green!20,
%%      cylinder end fill=green!20,
%      shape border rotate=90,
%      aspect=0.25,
%      draw
%    }
%  ]
%    \node[database] (defectont) at (0,0) {\shortstack{\DefectOnt\\Ontology}};
%    
%    
%    % MAM module
%    \node[database] (mam) at (0,-3) {\shortstack{\emph{MAM}\\\emph{4DefectOnt}}};
%    %
%    \node[database, align=center] (defectcore) at (-6,-6)
%    {
%    \emph{DefectCore} \\ \emph{4DefectOnt}
%    };
%%    \node[rectangle, rounded corners, draw, align=center] (defectcore) at (-6,-6)
%%{
%%    \emph{DefectCore}
%%    \\
%%    \emph{4DefectOnt} \\
%%    \rule[0.5ex]{2.5cm}{0.75pt} \\
%%\begin{varwidth}{3cm}
%%\begin{flushleft}
%%%\begin{enumerate}[leftmargin=0cm,noitemsep,topsep=0pt,label=$\cdot$]
%%%\item
%%$\cdot$
%%{\sf Defect}\\
%%$\cdot$
%%{\sf InducedDefect}\\
%%%\item
%%$\cdot$ \ldots
%%\end{flushleft}
%%%\end{enumerate}
%%\end{varwidth}
%%};
%        \node[database, align=center] (nist) at (-2,-6)
%        {
%        \emph{NIST} \\ \emph{4DefectOnt}
%        };
%%        \node[rectangle, rounded corners, draw, align=center] (nist) at (-2,-6)
%%        {
%%        \emph{NIST} \\ \emph{4DefectOnt} \\
%%    \rule[0.5ex]{2.75cm}{0.75pt} \\
%%\begin{varwidth}{3cm}
%%%\begin{enumerate}[leftmargin=0cm,noitemsep,topsep=0pt,label=$\cdot$]
%%%\item
%%$\cdot$ {\sf Characteristic} \\
%%%\item
%%$\cdot$ \ldots
%%%\end{enumerate} \\
%%\end{varwidth}
%%    };
%		\node[database, align=center] (mason) at (2,-6)
%	    {
%        \emph{MASON} \\ \emph{4DefectOnt}
%        };
%%		\node[rectangle, rounded corners, draw, align=center] (mason) at (2,-6)
%%	       {
%%        \emph{MASON} \\ \emph{4DefectOnt} \\
%%    \rule[0.5ex]{2.75cm}{0.75pt} \\
%%\begin{varwidth}{3cm}
%%%\begin{enumerate}[leftmargin=0cm,noitemsep,topsep=0pt,label=$\cdot$]
%%%\item
%%$\cdot$ {\sf Entity} \\
%%%\item
%%$\cdot$ \ldots
%%%\end{enumerate} \\
%%\end{varwidth}
%%    };
%		\node[database, align=center] (onto4add) at (6,-6) 
%		{
%		\emph{ONTO4ADD} \\ \emph{4DefectOnt}
%		};
%%		\node[rectangle, rounded corners, draw, align=center] (onto4add) at (6,-6) 
%%		{
%%		\emph{ONTO4ADD} \\ \emph{4DefectOnt}
%%		\\
%%	    \rule[0.5ex]{3cm}{0.75pt}
%%	    \\
%%	    \begin{varwidth}{3cm}
%%	    $\cdot$ {\sf PhysicalObject} \\
%%	    $\cdot$ \ldots
%%	    \end{varwidth}
%%		};
%		%
%%		    \node[box,draw] (n1) at (-6,-7) {some text};
%    %
%    \draw[->] (defectont) -- (mam);
%    \draw[->] (mam) -- (defectcore);
%    \draw[->] (mam) -- (nist);
%    \draw[->] (mam) -- (mason);
%    \draw[->] (mam) -- (onto4add);
%    
%    
%% Spatial module
%    \node[database] (spatial) at (0,3) {\shortstack{\emph{Spatial}\\\emph{4DefectOnt}}};
%    %
%        \node[database, align=center] (geosparql) at (-2,6) {\emph{GeoSPARQL} \\ \emph{4DefectOnt}};
%        \node[database, align=center] (mason2) at (2,6) {\emph{MASON} \\ \emph{4DefectOnt}};
%%    \node[rectangle, rounded corners, draw] (geosparql) at (-2,6) {\shortstack{\emph{GeoSPARQL} \\ \emph{4DefectOnt}}};
%%        \node[rectangle, rounded corners, draw] (mason2) at (2,6) {\shortstack{\emph{MASON} \\ \emph{4DefectOnt}}};
%    %
%    \draw[->] (defectont) -- (spatial);
%    \draw[->] (spatial) -- (geosparql);
%    \draw[->] (spatial) -- (mason2);
%    
%    
%    
%% Measure module
%    \node[database, align=center] (measure) at (3,0) {\emph{Measure}\\\emph{4DefectOnt}};
%    %
%        \node[database, align=center] (om) at (6,0) {\emph{OM4ExtruOnt} \\ \emph{4DefectOnt}};
%    %
%    \draw[->] (defectont) -- (measure);
%    \draw[->] (measure) -- (om);
%
%
%
%% Sensor module
%    \node[database, align=center] (sensor) at (-3,0) {\emph{Sensor}\\\emph{4DefectOnt}};
%    %
%    \node[database, align=center] (ssn) at (-6,0) {\emph{SSN} \\ \emph{4DefectOnt}};
%    %
%    \draw[->] (defectont) -- (sensor);
%    \draw[->] (sensor) -- (ssn);
%
%
%
%  \end{tikzpicture}
%	\caption{Diagram of the direct import structure for \emph{DefectOnt} modules with the corresponding signatures.\todo[inline]{\AM{Figures to discuss/fix}}}
%	\label{fig:mainclasses}	
%\end{figure}


%\begin{figure*}[h!]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/amdefectont.png}
%	\caption{Graphical representation of the \emph{DefectOnt} modules.}
%	\label{fig:mainclasses}	
%\end{figure*}


==> ArXiv/main/sec_ontomodule_am.tex <==
\subsection{\emph{MAM4DefectOnt} Module}
\label{sec:AM-mod}

==> ArXiv/main/sec_ontomodule_am_defectcore.tex <==

\noindent
%\subsubsection{\textnormal{\emph{defectcore4defectont}}}
The \emph{MAM4DefectOnt} module is the primary module of \emph{DefectOnt} ontology. This module consists of
three
%four
submodules:
\begin{enumerate*}[label=(\arabic*)]
%\emph{defectcore4defectont},
	\item\label{item:nistmodule}\emph{NIST4DefectOnt},
	\item\label{item:ontomodule}\emph{ONTO4ADD4DefectOnt},
	and
	\item\label{item:spatialmodule}\emph{Spatial4DefectOnt}.
\end{enumerate*}
%The former is
%a
%%\emph{ad hoc}
%newly
%developed module
%formalising domain knowledge about MAM defects,
%%involving ${\sf Defect}$ as main class,
%whereas the others
%These modules
%are
Modules~\ref{item:nistmodule} and~\ref{item:ontomodule} are obtained from the NIST AM ontology and the Onto4Additive ontology, respectively.
Module~\ref{item:spatialmodule} in turn consists of the following submodules:
\emph{GeoSPARQL4DefectOnt}, derived from GeoSPARQL1.1,
and
\emph{MASON4DefectOnt}, from
the MASON ontology.
%proposed by Sanfilippo,
In the following we present and discuss the relevant axioms of the \emph{MAM4DefectOnt} module, focusing on
the representation of
%its two main classes of {\sf Defect}, used to represent
the different types and sources of MAM defects analysed in the literature.
%and {\sf InducedDefect}, to model sources of defects.
%Moreover it inherits axioms and classes from a broader AM ontology, the NIST AMOntology. 
%\todo[inline]{\MC{Add paragrafo sul processo di reasoning e assioma fondamentale, vedi sotto. \AM{Ho pensato di spostare (e indebolire, perche' mi sembrava sostenesse qualcosa di troppo forte che non mi convinceva: poi te ne parlo) il paragrafo esplicativo del meccanismo di base della nostra ontologia nella Sec. 3 su Ontology Design and Development, perche' mi sembra che -- dato il suo carattere di osservazione generale, riguardante obiettivi e funzionamento -- stia meglio al di fuori della descrizione dei singoli moduli}}}

%To better explain the reasoning procedure we require from \emph{defectont}, let us consider a simple, yet explicative example:
%During a 3D printing process the monitoring system detects a feature $d$ which is classified -- by means of e.g., a pre-trained convolutional neural network -- as a porosity defect. At the same time, the system controller -- based on e.g., a reinforcement learning mechanism -- modifies the laser scanning speed to mitigate the propagation of the feature $d$. Starting from this set of online data, low-level reasoning mechanisms are not able to infer any causal relationship among laser scanning speed and the porosity defect. Contrary, our proposed ontology would be able to perform a high-level reasoning procedure establishing that the detected feature $d$ is a defect induced by laser parameters and scan strategy. 
%
%With such an objective in mind, in the following we introduce a set of axioms, classes, and properties able to construct an ontology suitable to infer from measured data the source of defects and, in the last instance, to shed light on the complex process-structure-property relationships occurring in MAM.

%Facciamo un esempio concreto. Supponiamo di scoprire in fase di stampa che una Feature $d$ osservata e' un $(i)$ PorosityDefect che e' $(ii)$ influencedBy some ScanningSpeed value: possiamo assumere di scoprire queste cose grazie a un sistema di controllo dei sensori basato su tecniche di machine learning, in grado di $(i')$ classificare un'immagine con una certa accuratezza come un caso di porosity e $(ii')$ aggiustare la scanning speed, sulla base di quanto appreso in fase di training, rilevando contestualmente una riduzione della porosity.
%Dato che nella nostra ontologia abbiamo ScanningSpeed $\sqsubseteq$ ProcessParameter, possiamo concludere che la Feature $d$ e' influencedBy some ProcessParameter.
%Assumendo che la nostra ontologia contenga anche l'assioma che asserisce
%%
%{\small{
%\[
%\hspace{-1cm}
%\text{ParameterAndScanStrategyInducedDefect $\equiv$ Defect $\sqcap$ influencedBy some ProcessParameter,}
%\]
%}}
%%
%possiamo concludere che la Feature $d$ e' un ParametersAndScanStrategyInducedDefect.
%Inoltre, assumendo che la nostra ontologia asserisca anche, seguendo la classificazione di Grasso e Colosimo, che
%{\small{
%\[
%\hspace{-2.5cm}
%\text{ProcessInducedDefect $\equiv$ ParameterAndScanStrategyInducedDefect $\sqcup$ ByproductAndMaterialEjectionInducedDefect},
%\]
%}}
%possiamo derivare che la Feature $d$ e' un ProcessInducedDefect.
%
%(Eventualmente -- ma questa e' la parte che adesso mi sembra ridondante -- se avessimo nella nostra ontologia anche che
%{\small{
%\[
%\text{ProcessInducedDefect $\sqsubseteq$ Defect $\sqcap$ hasSource some ProcessSource}
%\]
%}}
%potremmo inferire che $d$ e' un PorosityDefect che hasSource some ProcessSource).


%{\color{red}{
%TODO discuss -- Al momento, in molti casi, diciamo che un Defect ha come DefectSource di un certo tipo solo certi tipi di DefectSource, e che e' influencedBy solo da qualcosa. Asseriamo poi che molte DefectSource sono influencedBy solo da qualcosa. Ad esempio, un CrackingAndDelaminationDefect (fra le altre cose) ha come DesignSource solo SupportSource, ha come ProcessSource solo ParameterAndScanStrategySource, ed e' influencedBy solo da Shrinkage. Poi asseriamo che ParameterAndScanStrategySource e' influencedBy solo da 
%    HatchingDistance o HeatSourcePower o LayerThickness or PowderBedFusionProcessParameter o ScanningSpeed.
%    
%(1) Come prima opzione, propongo di modificare questi assiomi in modo da fare un uso piu' uniforme di `{\sf influencedBy}'. Mi sembra infatti ragionevole che un Defect possa essere influencedBy direttamente da certe proprieta' (come lo Shrinkage), ma che possa anche ``ereditare'' il fatto di essere influencedBy dalla propria DefectSource: ossia, se un Defect e' tale che hasSource qualche DefectSource, la quale a sua volta e' influencedBy qualcos'altro, allora quel Defect e' anch'esso stesso influencedBy quel qualcos'altro. Questa modifica potrebbe essere fatta nel modo seguente.
%\begin{itemize}
%\item Eliminare `{\sf influencedBy} {\tt only} {\sf Shrinkage}' da {\sf CrackingDelaminationDefect} e altri;
%\item Modificare assiomi dalla forma
%\[
%\bigwedge_{{\sf i} \in I} ( {\sf XDefect} \sqsubseteq  {\sf hasY}_{{\sf X}_{i}}{\sf Source} \ {\tt only} \ {\sf Z}_{{\sf X}_{i}}{\sf Source} )
%\
%\land
%\
% {\sf influencedBy} \ {\tt only} \ {\sf Influence}
%\]
%alla forma
%\[
% {\sf XDefect}
% \sqsubseteq
% \bigsqcup_{i \in I}
% ({\sf hasY}_{{\sf X}_{i}}{\sf Source} \ {\tt some} \ {\sf Z}_{{\sf X}_{i}}{\sf Source})
% \
% \sqcup
% \
% {\sf influencedBy} \ {\tt some} \ {\sf Influence}
%\]
%aggiungendo inoltre assiomi della forma
%\[
%{\sf hasSource} \circ {\sf influencedBy} \sqsubseteq {\sf influencedBy}
%\]
%\end{itemize}
%
%(2) La Proposta (1), comunque, non mi sembra ottimale. Forse e' anche metafisicamente poco chiara, perche' sembra dare priorita' concettuale alla relazione `avere come causa', rispetto alla relazione `essere influenzato da'. Invece, credo che il meccanismo inferenziale importante per noi, e che sta anche dietro alla classificazione dei difetti di Grasso e Colosimo, sia piu' o meno il seguente:
%\begin{itemize}
%\item supponiamo, in fase di stampa, di scoprire che una Feature   $d$ e' un Defect ed e' influencedBy qualche Characteristic (ad esempio, perche' un sensore nota una certa discontinuita' che viene modificata cambiando un qualche parametro di stampa);
%\item nella nostra ontologia, assumiamo di asserire che qualche cosa e' un $C$-InducedDefect se e solo se e' un Defect che e' influencedBy qualche cosa che e' $C$;
%(inoltre, potremmo decidere di aggiungere alla nostra ontologia -- ma forse e' ridondante -- anche l'informazione che $(\ast)$ se qualcosa e' un $C$-InducedDefect, allora hasSource qualche $C$-RelatedSource);
%\item quindi, possiamo concludere che la Feature $d$ e' un $C$-InducedDefect (e, se aggiungiamo $(\ast)$, concludere anche che $d$ hasSource qualche $C$-RelatedSource; d'altra parte, adesso questa conclusione non mi pare che dica niente di piu' di `$d$ e' un $C$-InducedDefect').
%\end{itemize}
%
%In sostanza, seguendo quest'altro approccio e all'opposto di quello che facciamo attualmente, a partire dalla relazione `essere influenzato da' -- che possiamo osservare direttamente modificando dei parametri di stampa -- saremmo in grado di concludere qualcosa a proposito della relazione `avere come causa' (o, di fatto con un senso equivalente, `essere indotto da', come scrivono anche Grasso e Colosimo) -- che mi sembra invece una relazione con una portata vagamente piu' ``epistemica'' e meno ``osservativa'' di `essere influenzato da', dato che sembra aggiungere un elemento esplicativo/nomotetico, oltre a quello della correlazione empirica diretta.
%Al contrario (come facciamo attualmente), cioe' partire dalla relazione di `avere come causa' come prioritaria, e spiegare questa in termini della relazione di `essere influenzato da', mi sembra poco chiaro, perche' in qualche modo ``reifica'' la nozione di causa, che viene poi spiegata nei termini ancora piu' basilari di `essere influenzato da', che e' una relazione ``osservabile''. Ma a noi, concretamente, non capitera' mai di ``osservare'' prima una causa, per poi inferire che questa e' ``influenzata da'' qualcosa.
%Scusa, sto sproloquiando un po' a spanne, ma e' per cercare di chiarire le idee anche a me stesso.
%
%
%Inoltre, al posto di assiomi come 
%{\small{
%\[
%\hspace{-3cm}
%\text{PorosityDefect $\sqsubseteq$ hasProcessSource only (ByProductsAndMaterialEjectionSource $\sqcup$ ParameterAndScanStrategySource)}
%\]
%}}
%(che antepongono la relazione di `avere come causa', specializzandola in molte sotto-relazioni, alla relazione di `essere influenzato da'),
%assieme ad altri assiomi analoghi,
%potremmo dire semplicemente che
%\begin{align*}
%\text{PorosityDefect $\sqsubseteq$ influencedBy only \ } & \text{(BuildChamberParameter $\sqcup$ HeatSourcePower $\sqcup$}  \\
%& \text{LayerThickness  $\sqcup$ PackingDensity $\sqcup$} \\
%& \text{PowderSizeDistribution  $\sqcup$ ScanningSpeed $\sqcup$ \ldots)}
%\end{align*}
%dove i `\ldots' sono la disgiunzione di tutti gli altri fattori che possono influenzare un porosity defect.
%
%Nota che questo ha il vantaggio di alleggerire notevolmente le relazioni: non c'e' piu' bisogno di avere a priori tante relazioni di `hasSource' specializzate (`hasProcessSource', `hasDesignSource', \ldots); possiamo basare tutto sulla relazione di `influencedBy', lasciando che sia il ``ragionamento'' a farci concludere che tipo di origine ha il difetto, ossia da cosa e' indotto, a seconda del parametro che osserviamo avere un'influenza su di esso.
%}}


==> ArXiv/main/sec_ontomodule_am_defectcore_defect.tex <==
\subsubsection{Defect types in \emph{MAM4DefectOnt}}
%\subsubsection*{{\sf Defect} Class}
\label{sec:defecttype}
%
\noindent
The main class of the module used to represent the different kinds of MAM defects studied in the literature is the {\sf Defect} class (cf. Figure~\ref{fig:DefectOntomodules}).
On this class, we first impose the following constraint:
\begin{equation}
{\sf Defect} \sqsubseteq {\sf PhysicalObject} \sqcap \exists{\sf affects}.({\sf PhysicalArtefact} \sqcup {\sf Material}),
\end{equation}
where: {\sf PhysicalObject}, {\sf PhysicalArtefact}, and  {\sf Material} are classes in \emph{ONTO4ADD4DefectOnt}; {\sf affects} is a newly introduced object property, used to represent the relationship between a defect and a physical entity that is affected by it, having domain {\sf Defect}, range {\sf Physical} (from the \emph{NIST4DefectOnt} module), and inverse property {\sf isAffectedBy}.


\begin{figure}[t]
%	\includegraphics[width=\textwidth]{figures/DefectClassExploded.png}
	\includegraphics[width=\textwidth]{figures/defect_class.png}
	\caption{Main super- and sub-classes of the class ${\sf Defect}$ in \DefectOnt.}
	\label{fig:DefectOntomodules}	
\end{figure}


%\ldots\todo{\AM{todo add explanation}}

As a further step, we leverage the \emph{Spatial4DefectOnt} module imported by \emph{MAM4DefectOnt} to provide a location-based classification of defects.
First, we define a \emph{located defect} as a defect that overlaps with some region of an AM layer, as follows:
\begin{equation}
	{\sf LocatedDefect} \equiv {\sf Defect} \sqcap \exists {\sf sfOverlaps}.{\sf AMLayerRegion},
\end{equation}
where:
{\sf sfOverlaps} comes from the \emph{Spatial4DefectOnt} submodule,
%and it is
in turn obtained from GeoSPARQL1.1, where it represents the partially overlapping relation from the region connection calculus (RCC)~\cite{RanEtAl92};
and {\sf AMLayerRegion} is a newly introduced subclass of {\sf PhysicalRegion}, in turn set in \emph{MAM4DefectOnt} as subclass of {\sf PhysicalObject} from \emph{ONTO4ADD4DefectOnt}.
Moreover, we distinguish between \emph{internal defects} (i.e., defects located in overlapping with some infill regions, and with infill regions only, of an AM layer) and \emph{surface defects} (i.e., defects located so to overlap with contour regions of an AM layer).
The axioms formalising the above characterisation are the following:
\begin{align}	
	{\sf InternalDefect} \equiv \ & {\sf LocatedDefect} \sqcap \exists{\sf sfOverlaps}.{\sf InfillRegion} \sqcap \forall{\sf sfOverlaps}.{\sf InfillRegion}, \\
	{\sf SurfaceDefect} \equiv \ & {\sf LocatedDefect} \sqcap \exists{\sf sfOverlaps}.{\sf ContourRegion},
\end{align}
%\begin{align}	
%	{\sf InternalDefect} \equiv \ & {\sf Defect} \sqcap \exists{\sf sfOverlaps}.{\sf InternalAMLayer} \sqcap \forall{\sf sfOverlaps}.{\sf InternalAMLayer}, \\
%	{\sf SurfaceDefect} \equiv \ & {\sf Defect} \sqcap \exists{\sf sfOverlaps}.{\sf SurfaceAMLayer},
%\end{align}
together with the axioms stating that 	{\sf ContourRegion} and {\sf InfillRegion}, together with {\sf PowderRegion}, are disjoint subclasses of {\sf AMLayerRegion}, and ${\sf AMLayer} \sqsubseteq \exists {\sf hasPart}.{\sf AMLayerRegion}$.
%{\sf isLayerOf}
%%\todo{\AM{to discuss -- use {\sf partOf} from \emph{Onto4Add4DefectOnt} instead?}}
%is a property introduced in our \emph{MAM4DefectOnt} module, with {\sf isLayerOf} inverse of {\sf hasLayer} from \emph{ONTO4ADD4DefectOnt}.
%
%\begin{align}
%
%
%
%\end{align}

To formalise additional domain knowledge on MAM defects, we rely on the MAM defect classification proposed by Grasso and Colosimo in \cite{grasso2017process}. 
Due to its level of detail, this classification is preferred as the main reference framework over others in the AM literature (e.g., \cite{debroy2018additive,frazier2014metal,smith2016linking}). 
However, aiming at a broad and consistent representation model for MAM defects, we integrate in our ontology also other resources from the literature, adjusting where needed the overall structure of \citeauthor{grasso2017process} classification (cf. \autoref{sec:ont-design-meth}).
%However, in \emph{DefectOnt}, we do not strictly follow the categories and the definitions proposed in \cite{grasso2017process}, since they lack of rigorous, logically consistent definitions. In fact, the present work does not limit to formalize  knowledge already present in the literature, but instead it aims at introducing novel logical relationships able to construct a consistent domain knowledge representation of MAM defects.
%

In \cite{grasso2017process}, the MAM defects are organised in six
main categories, represented in our module by corresponding subclasses of the ${\sf Defect}$ class:
%principal groups:
\begin{enumerate*}[label=$(\roman*)$]
\item \emph{porosity} ({\sf PorosityDefect});
\item \emph{balling} ({\sf BallingDefect});
\item \emph{geometric defects} ({\sf GeometricDefect});
\item \emph{surface defects} ({\sf SurfaceRoughnessDefect});
\item \emph{cracks and delaminations} ({\sf CrackingDefect});
\item \emph{microstructural inhomogeneities and impurities} ({\sf MicrostructuralDefect}).
\end{enumerate*}
%We represent these groups in our ontology by corresponding subclasses of our {\sf Defect} class:
%(cf. Figure~\ref{fig:DefectOntomodules}),
%%\ref{fig:defetctmodule},
%namely: {\sf SurfaceDefect}, {\sf BallingDefect}, {\sf CrackingDefect}, {\sf GeometricDefect}, {\sf MicrostructuralDefect}, and {\sf PorosityDefect}.
We introduce the {\sf SurfaceDefect} and {\sf InternalDefect} class to model purely location-based notions of defects, with respect to the AM layers they overlap with. Therefore, we employ the class {\sf SurfaceRoughnessDefect} to represent the specific kind of surface defects affecting the roughness of a product surface, that~\citeauthor{grasso2017process} simply refer to as \emph{surface defects}.

In order to present the ontology axioms used to connect these classes of defects with their corresponding sources, as well as to formalise their relationships with other AM concepts, we report in the following the main features of each group of defects.












\paragraph{Balling defects}
%\todo[inline]{\MC{Nel NIST abbiamo una classe SurfaceTensionEffects che userei al posto di BallingEvent!!} \AM{Io vedo solo {\sf SurfaceTension} in NIST: intendi quella? In ogni caso direi che mi va bene.}}
The surface tension generated in the melt pool can lead to melted balls of liquid metal that solidify into spherical particles, generating the so-called \textit{balling} phenomenon. These small spheres of metal may affect both the internal layers of the product, as well as its surface,
%These small spheres of metals influence
influencing the component surface roughness and porosity, and (if the phenomenon is very pronounced) it may eventually lead to (hemi-)spherical protrusion on the solidified structure. Balling can have dramatic effects on part quality and fatigue life of the component \cite{malekipour2018common}. 
To translate the above description into logical axioms, we distinguish between {\sf InternalBallingDefect} and {\sf SurfaceBallingDefect}
as subclasses covering
%such that the union of these two (disjoint) classes forms
the {\sf BallingDefect} class, as follows:
%
%\todo[inline]{\MC{C'è un errore nella (2), riesci per favore a ricontrollare?} \AM{Mi sa che non abbiamo sistemato questa cosa di persona, ho improvvisato. Intanto dai un'occhiata, ne riparliamo.}}

\begin{align}
		\notag
		{\sf InternalBallingDefect} \equiv \
		\notag
		& {\sf InternalDefect} \ \sqcap \\
		\notag
		& \exists{\sf isConsequenceOf}.{\sf SurfaceTensionPhenomenon} \ \sqcap \\
		\notag
		& \exists{\sf isMadeOf}.({\sf Material} \sqcap \exists {\sf hasMaterialState}.\{ {\sf solidState} \})  \ \sqcap \\
%\notag
		& \exists {\sf hasApproximateGeometry}.{\sf Ball}, \\
		%
		\notag
		{\sf SurfaceBallingDefect} \equiv \
		& {\sf SurfaceDefect} \ \sqcap \\
		\notag
		& \exists{\sf isConsequenceOf}.{\sf SurfaceTensionPhenomenon} \ \sqcap \\
		\notag
		& \exists{\sf isMadeOf}.({\sf Material} \sqcap \exists {\sf hasMaterialState}.\{ {\sf solidState} \})  \ \sqcap \\
%\notag
		& \exists {\sf hasApproximateGeometry}.{\sf HemiBall}, \\
	{\sf BallingDefect} \equiv \ &
	{\sf InternalBallingDefect} \sqcup {\sf SurfaceBallingDefect},
%	{\sf InternalBallingDefect} \sqsubseteq \ & \lnot {\sf SurfaceBallingDefect} 
\end{align}
%\begin{align}
%		\notag
%	{\sf BallingDefect} \equiv \ & {\sf Defect} \sqcap \exists {\sf hasApproximateGeometry}.({\sf HemiBall} \sqcup {\sf Ball}) \ \sqcap \\
%				\notag
%	& \exists{\sf isMadeOf}.({\sf Material} \sqcap \exists {\sf hasMaterialState}.\{ {\sf solidState} \})  \ \sqcap
%\\
%	& \exists{\sf isConsequenceOf}.{\sf SurfaceTensionPhenomenon} \\
%%	{\sf InternalBallingDefect} \sqcup {\sf InternalBallingDefect}
%%	{\sf InternalBallingDefect} \sqsubseteq \ & \lnot {\sf SurfaceBallingDefect} 
%%		\notag
%		{\sf InternalBallingDefect} \equiv \ &
%%		{\sf BallingDefect} \sqcap
%%\notag
%		 {\sf InternalDefect} \sqcap {\sf BallingDefect}  \sqcap
%%		\notag
%%		& \forall{\sf affects}.{\sf InternalAMLayer} \ \sqcap \\
%%		\notag
%		\exists{\sf hasApproximateGeometry}.{\sf Ball} \\
%%		\notag
%%	& \exists{\sf isMadeOf}.({\sf Material} \sqcap \exists {\sf hasMaterialState}.\{ {\sf solidState} \})  \ \sqcap
%%\\
%%	& \exists{\sf isConsequenceOf}.{\sf SurfaceTensionPhenomenon} \\
%		%
%%		\notag
%		{\sf SurfaceBallingDefect} \equiv \ &
%%		{\sf BallingDefect} \sqcap
%%\notag
%		 {\sf SurfaceDefect}  \sqcap  {\sf BallingDefect} \sqcap
%%		\notag
%%		& \forall{\sf affects}.{\sf SurfaceAMLayer}  \ \sqcap \\
%%		\notag
%		\exists {\sf hasApproximateGeometry}.{\sf HemiBall}
%%				\notag
%%	& \exists{\sf isMadeOf}.({\sf Material} \sqcap \exists {\sf hasMaterialState}.\{ {\sf solidState} \})  \ \sqcap
%%\\
%%	& \exists{\sf isConsequenceOf}.{\sf SurfaceTensionPhenomenon} \\
%\end{align}
where:
{\sf isConsequenceOf} is a property introduced in our \emph{MAM4DefectOnt} module;
the property {\sf hasApproximateGeometry}, as well as the classes {\sf Ball} and {\sf HemiBall}, are introduced in \emph{Spatial4DefectOnt};
 {\sf SurfaceTensionPhenomenon} is set in \emph{MAM4DefectOnt}  as a subclass of {\sf Phenomenon}, in turn inherited from the \emph{NIST4DefectOnt} submodule;
{\sf isMadeOf} is an object property of \emph{MASON4DefectOnt};
while {\sf Material}, {\sf hasMaterialState}, and {\sf solidState} are, respectively, a class, a property and an individual taken from \emph{ONTO4ADD4DefectOnt}.
%{\sf madeOf} an object property taken from ONTO4ADD.
%
%{\color{red}{
%TODO discuss/add other axioms -- The idea is that we could use the ontology to formalise most of the experts' knowledge about defects: so far, we express what are their sources, and by what are they influenced; but what about what these defects actually are, i.e., how they are more or less defined, or what are their necessary properties? For instance, in the example below we characterise a balling defect as a defect that has the shape of a metal sphere, where `{\sf Sphere}' comes from EMMO (to be added?), `{\sf hasShape}' comes from MASON, and `{\sf hasMaterialState}' comes from onto4additive (where does `{\sf Solid}' come from?):
%{\small{
%\[
%\hspace{-2cm}
%{\sf BallingDefect} \sqsubseteq {\sf Defect} \ {\tt and} \ {\sf hasShape} \ {\tt some} \ ({\sf Sphere} \ {\tt and} \ {\sf madeOf}  \ {\tt some} \ ({\sf Metal} \ {\tt and} \ {\sf hasMaterialState} \ {\tt some} \ {\sf Solid}))
%\]
%}}
%}}













\paragraph{Cracking and delamination defects}
According to \cite{debroy2018additive} there are three main cracking mechanisms observed in MAM: $(i)$ solidification cracking along the boundaries, $(ii)$ liquation cracking occurring either in the mushy region or in the partially melted zone, and $(iii)$ delamination, consisting in the separation of two consecutive printed layers. All the three types of cracking are related to the high residual stresses induced by the process \cite{mercelis2006residual} as a consequence of stress relief through fracture. This characterising feature of cracking defects is formalised in our ontology as follows:
%
\begin{align}
\notag
{\sf CrackingDefect} \equiv \ & {\sf Defect} \ \sqcap \\
\notag
& \exists{\sf affects}.({\sf AMProduct} \ \sqcap \\
& \exists{\sf hasFeature}.(\exists{\sf isConsequenceOf}.{\sf Fracture}))
\end{align}
%
with: {\sf hasFeature} object property of \emph{ONTO4ADD4DefectOnt};
and class {\sf Fracture} introduced in \emph{MAM4DefectOnt} within the subclass hierarchy of {\sf Phenomenon} from \emph{NIST4DefectOnt}.
In our module, we also introduce specific subclasses for each type of cracking, in order to better specialise their relationship with the process, namely: {\sf SolidificationCrackingDefect}, {\sf LiquationCrackingDefect}, and {\sf DelaminationCrackingDefect}.
%
%{\color{red}{
%TODO discuss/add other axioms (cf. e.g. Balling) -- In particular
%{\small{
%\[
%\text{SolidificationCrackingDefect $\sqsubseteq$ CrackingDelaminationDefect}
%\]
%\[
%\text{LiquationCrackingDefect $\sqsubseteq$ CrackingDelaminationDefect}
%\]
%\[
%\text{DelaminationDefect $\sqsubseteq$ CrackingDelaminationDefect}
%\]
%}}
%and some axiom to formalise:
%\begin{center}
%disconnection of parts ``as a consequence of a stress relief through fracturing when the tensile stress exceeds the ultimate tensile strength of the solid material at a given point and temperature''~\cite{grasso2017process}
%\end{center}
%}}
%













\paragraph{Geometric defects}
%\todo[inline]{\MC{In MASON abbiamo una classe Shape subclass di GeometricEntity che userei al posto di Geometry. \AM{Ok.}}}
This class of defects includes all the different kinds of dimensional and geometric deviations from the original, as-designed geometry \cite{malekipour2018common}.
In fact, it is widely documented in the literature that complex, lattice, and slender 3D printed structures present non negligible geometric deviation from the the actual, as-build structure and the as-design geometry as generated within Computer Aided Design (CAD) environments \cite{korshunova2021bending,BONIOTTI2019105181,KORSHUNOVA2021101949}. Such kind of defects is defined in the \emph{MAM4DefectOnt} module, as follows:
%
\begin{align}
		\notag
		{\sf GeometricDefect} \equiv \ & {\sf Defect} \ \sqcap \\
		\notag
		& \exists {\sf affects}.({\sf AMProduct} \sqcap \exists{\sf hasGeometry}.({\sf AsBuiltGeometry} \ \sqcap \\
		& \exists{\sf hasSignedDeviationFrom}.{\sf AsDesignedGeometry})),
\end{align}
%\begin{align}
%		\notag
%		{\sf GeometricDefect} \equiv \ & {\sf Defect} \sqcap \\
%		\notag
%		& \exists {\sf affects???}.({\sf PhysicalArtefact???} \sqcap \exists{\sf hasGeometry}.({\sf AsBuiltGeometry???} \sqcap \\
%		& \lnot \exists{\sf sameAs???}.{\sf AsDesignedGeometry???}))
%\end{align}
%\todo[inline]{\MC{Ma dire che PhysicalObject has (Shape etc...)? In modo da non introdurre una nuova classe...}\AM{Ok, ma va bene usare {\sf hasGeometry} da GeoSPARQL, che e' meno vago di {\sf has}?}}
%\todo[inline]{\MC{Proposta sostituire: hasSignedDeviationFrom->not sameAs, con sameAs preso dal NIST} \AM{Purtroppo direi che non e' esprimibile nella logica che abbiamo a disposizione}}
%
where:
{\sf hasGeometry} and {\sf hasSignedDeviationFrom} are properties, and {\sf AsBuiltGeometry} and {\sf AsDesignedGeometry} are classes introduced in the \emph{Spatial4DefectOnt} module.

The most common effects leading to geometric defects are: $(i)$ shrinkage, $(ii)$ warping, $(iii)$ curling, and $(iv)$ formation of super-elevated edges. They are inserted into the module as subclasses of {\sf GeometricDefect} and defined as: {\sf ShrinkageGeometricDefect}, {\sf WarpingGeometricDefect}, {\sf CurlingGeometricDefect}, {\sf SuperelevatedEdgesGeometricDefect}, respectively.
%
\paragraph{Microstructural defects}
Several different classifications can be found in MAM literature to label and classify the defects related to the microstructure of 3D printed components \cite{MIKULA2021109851,song2015differences}. 
For our purposes, to provide an axiom characterising microstructural defects, we first introduce in \emph{MAM4DefectOnt} the class {\sf InhomogeneousMicrostructure} as a subclass of {\sf Microstructure}, that we inherit from the
NIST ontology.
%\emph{nist4defectont} module.
The axiom formalising that a microstructural defect is any defect that affects an AM product with inhomogeneous microstructure is then written as follows:
%
\begin{align}
\notag
	{\sf MicrostructuralDefect} \equiv \ & {\sf Defect} \sqcap \exists{\sf affects}.({\sf AMProduct} \ \sqcap \\
%	& \exists{\sf hasCharacteristic}
	& \exists{\sf presents}.{\sf InhomogeneousMicrostructure})
\end{align}
%To define an axiom describing microstructural defects, we need to introduce the concept of inhomogeneous microstructure as a subclass of {\sf Microstructure}, a class that we inherit from the
%NIST ontology.
%%\emph{nist4defectont} module.
%Thus, the two axioms defining {\sf InhomogeneousMicrostructure} and {\sf MicrostructuralDefect}, respectively can be written as follows:
%%
%\begin{align}
%	{\sf InhomogeneousMicrostructure} \sqsubseteq \ & {\sf Microstructure}
%	\\
%	\notag
%	{\sf MicrostructuralDefect} \equiv \ & {\sf Defect} \sqcap \exists{\sf affects}.({\sf AMProduct} \ \sqcap \\
%	& \exists{\sf hasCharacteristic}.{\sf InhomogeneousMicrostructure})
%\end{align}
%
where
{\sf presents} is a newly introduced object property in \emph{MAM4DefectOnt}, used to relate physical objects with the characteristics they exhibit.
%{\sf hasCharacteristic}
%%and {\sf Microstructure} are, respectively,
%is an object property
%%and a class
%from the NIST AM ontology. 
%while {\sf InhomogeneousMicrostructure} is a newly introduced subclass of the latter. 
%We would like to remark that, to maintain a uniform naming scheme, in our module \emph{NIST4DefectOnt} we replace the IRI of the original NIST AM class {\sf Inhomogenity} with {\sf InhomogeneousMicrostructure}.
%\todo{\AM{non trovo piu' {\sf Inhomogenity} in NIST}}
%\todo[inline]{\AM{todo add comment on terminology change {\sf Inhomogenity} (NIST) $\to$ {\sf InhomogeneousMicrostructure} }}
Finally, following \citet{sharratt2015non}, we distinguish between three types of inhomogeneities of the microstructure that occur during MAM processes, introducing them as corresponding subclasses of {\sf MicrostructuralDefect}: $(i)$ impurities ({\sf ImpuritiesMicrostructuralDefect}), $(ii)$ grain size characteristics ({\sf GrainSizesMicrostructuralDefect}), and $(iii)$ crystallographic textures ({\sf CrystallographicTexturesMicrostructuralDefect}).
%Finally, to determine the subclasses of the ${\sf MicrostructuralDefect}$ class we refer to \cite{sharratt2015non}. In particular, we consider three types of inhomogeneities of the microstructure occurring during MAM processes: $(i)$ impurities, $(ii)$ grain size characteristics, and $(iii)$ crystallographic textures, that we introduce as three corresponding subclasses of {\sf MicrostructuralDefect}, namely: {{\sf ImpuritiesMicrostructuralDefect}, {\sf GrainSizesMicrostructuralDefect}, and \sf CrystallographicTexturesMicrostructuralDefect}, respectively.
% 









\paragraph{Porosity defects}
Fully dense (99.95$\%$) MAM parts can be produced when printing large bulk material components. However, more often a functional design and/or lightweight structures (e.g., lattice) are present in MAM products (cf.~\cref{fig:poresPic}). In this case porosity -- due, e.g, to lack-of-fusion or keyhole effects -- can severely affect the performances of 3D printed components. Based on the location of the defects, 
%\todo{\AM{todo explain}}
%%{\sf TwoManifold}, {\sf Compact}, and {\sf isBoundaryOf}.
%Moreover,
we further specify the notions of \emph{internal} and \emph{surface} porosity defects (cf. Figure~\ref{subfig:smallPores} and~\ref{subfig:largePores}, respectively), formalising them respectively as {\sf InternalPorosityDefect} and {\sf SurfacePorosityDefect},
%so to cover {\sf PorosityDefect}
as follows:
%
\begin{align}	
%		\notag
		{\sf InternalPorosityDefect} \equiv \ & {\sf InternalDefect} \sqcap {\sf VoidRegion} \sqcap \exists{\sf hasBoundary}.{\sf ClosedSurface} \\
%		\notag
		{\sf SurfacePorosityDefect} \equiv \ & {\sf SurfaceDefect} \sqcap {\sf VoidRegion} \\
%	\begin{split}
%		&{\sf PorosityDefect} \sqsubseteq {\sf Defect} \sqcap \exists{\sf hasApproximateGeometry}.\\
%		& ({\sf TwoManifold} \ {\tt and} \ {\sf Compact} \ {\tt and} \ {\sf isBoundaryOf}  \ {\tt some} \  {\sf Void})
%	\end{split}
		{\sf PorosityDefect} \equiv \ & {\sf SurfacePorosityDefect} \sqcup {\sf InternalPorosityDefect}
\end{align}
%\begin{align}	
%		\notag
%		{\sf InternalPorosityDefect} \equiv \ & {\sf PorosityDefect} \sqcap {\sf InternalDefect} \sqcap \forall {\sf affects}.{\sf InternalAMLayer} \ \sqcap \\
%		& \exists{\sf hasGeometry}.({\sf ClosedSurface} \sqcap \exists{\sf isBoundaryOf}.{\sf VoidRegion}) \\
%		\notag
%		{\sf SurfacePorosityDefect} \equiv \ & {\sf PorosityDefect} \sqcap {\sf SurfaceDefect} \sqcap \forall {\sf affects}.{\sf SurfaceAMLayer} \ \sqcap \\
%		& {\sf VoidRegion} \\
%%	\begin{split}
%%		&{\sf PorosityDefect} \sqsubseteq {\sf Defect} \sqcap \exists{\sf hasApproximateGeometry}.\\
%%		& ({\sf TwoManifold} \ {\tt and} \ {\sf Compact} \ {\tt and} \ {\sf isBoundaryOf}  \ {\tt some} \  {\sf Void})
%%	\end{split}
%		{\sf PorosityDefect} \equiv \ & {\sf SurfacePorosityDefect} \sqcup {\sf InternalPorosityDefect}
%\end{align}
%
where:
{\sf isBoundaryOf} and {\sf ClosedSurface} are, respectively, a property and a class introduced in \emph{Spatial4DefectOnt};
${\sf VoidRegion}$ is a newly introduced class (cyclically) defined in \emph{MAM4DefectOnt} as
${\sf VoidRegion} \equiv {\sf PhysicalObject} \ \sqcap \  \forall {\sf hasPart}.{\sf VoidRegion}$.
%defined in
%\emph{NISTAM4DefectOnt} as a subclass of {\sf ProcessSignature} as in NIST AM ontology.
%\todo[inline]{\AM{${\sf VoidRegion} \equiv {\sf PhysicalObject} \sqcap \forall {\sf hasPart}.{\sf VoidRegion}$}}

%\todo[inline]{\AM{remove Figure~\ref{fig:poresPic}?}}


\begin{figure}[h!]
	\centering
	\subfloat[Internal porosity defect.\label{subfig:smallPores}]
	{
		\includegraphics[width=0.458\textwidth]{figures/smallPores.jpg}
	}
	\subfloat[Surface porosity defect.\label{subfig:largePores}]
	{
		\includegraphics[width=0.4\textwidth]{figures/largePores.png}
	}    
	\caption{View by micro-Computed Tomography showing different kinds of pores in a Stainless Steel 316L 3D printed specimen~\cite{carraturo2021experimental}.}
	\label{fig:poresPic}
\end{figure}
%









\paragraph{Surface roughness defects}
%
Surface roughness defects are clearly related to the notion of surface roughness, i.e., to a deviation of the surface texture with respect to an ideal surface plane. In MAM processes, surface roughness is influenced by two main effects: the stair-stepping effects, due to the layer-by-layer nature of the process, and the actual roughness of the metal surface \cite{fox2016,strano2013surface}. Additionally, the relative position of the surface strongly influences its roughness, e.g., downward surfaces present much higher roughness than upward surfaces.
We formalise the connection between surface roughness defects and the rough surface texture of a product, as follows:
%\todo{
%\AM{
%changed, to check!
%}}
%\todo[inline]{\MC{Add missing classes and properties in Protege!! Rimuovere hasSource da defectcore}}
\begin{align}
		\notag
		{\sf SurfaceRoughnessDefect} \equiv \ & {\sf SurfaceDefect}  \ \sqcap \\
		& \exists {\sf affects}.({\sf AMProduct} \sqcap
		\exists{\sf presents}.{\sf RoughSurfaceTexture})
%		\exists{\sf hasCharacteristic}.{\sf RoughSurfaceTexture})
\end{align}
where:
{\sf AMProduct} is a class from the \emph{ONTO4ADD4DefectOnt} module; and {\sf RoughSurfaceTexture} is introduced as subclass of {\sf SurfaceTexture} in \emph{MAM4DefectOnt}.


%We also introduce the following additional subclasses
%\begin{align}
%	{\sf ProperInternalDefect} \equiv \ & {\sf InternalDefect} \sqcap \forall {\sf affects}.{\sf InternalAMLayer} \\
%	{\sf ProperSurfaceDefect} \equiv \ & {\sf SurfaceDefect} \sqcap \forall {\sf affects}.{\sf SurfaceAMLayer}
%\end{align}
%requiring them to affect only internal or surface layers, respectively.


==> ArXiv/main/sec_ontomodule_am_defectcore_induceddefect.tex <==
%
\subsubsection{Defect sources in \emph{MAM4DefectOnt}}
%\subsection*{{\sf InducedDefect} class}
\label{sec:defectsource}

\noindent
In order to establish logical connections between MAM defects and their causes,
%To correctly perform high-level reasoning able to establish logical relationships among defects and their source,
a further classification of defects based on the corresponding sources is required.
To this goal, we introduce {\sf InducedDefect} as a subclass of {\sf Defect}, defining it as follows:
%\todo{\MC{only or some?}}
\begin{align}	
\notag
		{\sf InducedDefect} \equiv \ & {\sf Defect} \sqcap \exists{\sf isInducedBy}.({\sf Characteristic} \sqcup  {\sf Material} \ \sqcup \\
		& {\sf Phenomenon} \sqcup {\sf PhysicalObject} \sqcup  {\sf Process})
%		\sqcup {\sf Defect})} 
\end{align}
where the newly introduced object property {\sf isInducedBy} represents the relationship between defects and those MAM entities that are known to have an influence on them.
%To model subclasses of {\sf InducedDefect}, we rely again on the classification proposed by \citet{grasso2017process}, that we further extend and specify. 
%According to the authors,
According to the classification proposed by \citet{grasso2017process}, Table~1 (and references therein), that we further extend and specify,
MAM defect sources are classified into four main groups, for which we introduce a corresponding  subclass of {\sf InducedDefect}:
\begin{enumerate*}[label=$(\roman*)$]
%\ref{fig:defetctsourcemodule}
	\item \emph{design for additive choices} ({\sf DesignInducedDefect});
	\item \emph{equipment} ({\sf EquipmentInducedDefect});
	\item \emph{feedstock material} ({\sf FeedstockMaterialInducedDefect}); and 
	\item \emph{process} ({\sf ProcessInducedDefect}). 
\end{enumerate*}
%For each of these defect sources, we introduce a corresponding induce defect subclass, that is:
%$(i')$ {\sf DesignInducedDefect}; 
%$(ii')$  {\sf EquipmentInducedDefect};
%$(iii')$ {\sf FeedstockMaterialInducedDefect}; and 
%$(iv')$ {\sf ProcessInducedDefect}. 
%
%Our goal is to model the relationships between such categories of induced defects and those process features that are known to have an influence on them.
%To do so, we rely on
%axioms that characterise each of the {\sf InducedDefect} subclasses, by means of
%the newly introduced object property
%{\sf isInducedBy}.
%%{\sf isInducedBy} as an object property.
%%paving the way towards an explainable online control of MAM processes based on high-level reasoning mechanisms.
In the following, we discuss the axioms that characterise each of the {\sf InducedDefect} subclasses.
%Moreover,
%%following~\citet{grasso2017process}, Table~1 (and references therein),
%we discuss the mappings connecting
%types of defects
%%each subclass of {\sf Defect}
%formalised in Section~\ref{sec:defecttype} with the corresponding causes identified in the literature.
%%presenting them as subclasses of {\sf InducedDefect}.
%Such mappings take the form of subsumption axioms $C \sqsubseteq D$, where: $C$ is any of the classes {\sf BallingDefect}, {\sf CrackingDefect}, {\sf GeometricDefect}, {\sf MicrostructuralDefect}, {\sf PorosityDefect}, {\sf SourfaceRoughnessDefect}; and $D$ is a union of subclasses of {\sf InducedDefect}.





% 
\paragraph{Design-induced defects}
A wrong support design and/or part orientation during the building process can have a dramatic impact on the part quality and performances of 3D printed components. In fact, these two parameters directly influence $(i)$ dimensional accuracy, $(ii)$ surface roughness, and $(iii)$ part microstructure \cite{kleszczynski2012error,foster2015optical,zeng2015optimization,strano2013surface}.
Accordingly, in the \emph{MAM4DefectOnt} module the class {\sf DesignInducedDefect} includes two other classes, {\sf SupportsInducedDefect} and {\sf OrientationInducedDefect}, defined by the following axioms:
%
\begin{align}	
		{\sf SupportsInducedDefect} \equiv \ & {\sf DesignInducedDefect} \sqcap \exists{\sf isInducedBy}.{\sf AMSupportStructure} 
\\
	{\sf OrientationInducedDefect} \equiv \ & {\sf DesignInducedDefect} \sqcap \exists{\sf isInducedBy}.{\sf ProductOrientation}
%	 {\sf DesignInducedDefect}  \equiv \ & {\sf SupportInducedDefect} \sqcup {\sf OrientationInducedDefect}
\end{align}
where {\sf AMSupportStructure} comes from \emph{ONTO4DD4DefectOnt}, while {\sf ProductOrientation} is a new subclass of {\sf ProductCharacteristic} introduced in \emph{MAM4DefectOnt}.






%
\paragraph{Equipment-induced defects}
Improper or sub-optimal setting and calibration of the MAM equipment can generate several types of defects. This category includes four main sources of defects:
$(i)$ beam scanning and deflection system;
$(ii)$ powder handling and deposition system;
$(iii)$ insufficient baseplate thickness;
and 
$(iv)$ build chamber environmental control (e.g., preheating of the powder bed) \cite{foster2015optical,kleszczynski2012error,prabhakar2015computational,spears2016process}. Each of these sources can be linked to different types of defects. For instance, an erroneous calibration of the beam scanning can lead to longer exposure time distorting the melt pool morphology, which directly affects residual stresses, geometric accuracy, and porosity (lack of fusion defects) in the final component \cite{yeung2016,marques2020numerical,vastola2016modeling,carraturo2020numerical}.
In the \emph{MAM4DefectOnt} module, we introduce the class {\sf EquipmentInducedDefect} that, in accordance with the observations above, includes four subclasses: {\sf BaseplateInducedDefect}, {\sf BeamScanningDeflectionSystemInducedDefect}, {\sf BuildChamberEnvironmentalControlInducedDefect}, and {\sf PowderHandlingDepositionSystemInducedDefect}.
In turn, these are defined by the following axioms:
%
%{\footnotesize
\begin{align}	
		\notag
		{\sf EquipmentInducedDefect} \equiv \ & {\sf InducedDefect} \ \sqcap \ \\
		\notag
		& \exists{\sf isInducedBy}.({\sf EquipmentParameter} \ \sqcup \\
		\notag
		& {\sf MfgDevice} \ \sqcup \\
		& ({\sf Material} \sqcap \exists {\sf makes}.{\sf MfgDevice})) \\
		\notag
		{\sf BaseplateInducedDefect} \equiv \ & {\sf EquipmentInducedDefect} \ \sqcap \ \\
		\notag
		& \exists{\sf isInducedBy}.({\sf BaseplateMaterial} \ \sqcup  \\
		\notag
		& {\sf BaseplatePreHeatingTemperature} \ \sqcup \\
		& {\sf BaseplateThickness}) \\
		\notag
		{\sf BeamScanningDeflectionSystem} \phantom{\ \equiv \ } & \\
		\notag
		{\sf InducedDefect} \equiv \ & {\sf EquipmentInducedDefect} \ \sqcap \\
		& \exists{\sf isInducedBy}.{\sf OpticalParameter}	\\
		\notag
		{\sf BuildChamberEnvironmentalControl} \phantom{\ \equiv \ } & \\
		\notag
		{\sf InducedDefect} \equiv \ & {\sf EquipmentInducedDefect} \	\sqcap \\
		& \exists{\sf isInducedBy}.{\sf BuildChamberParameter} \\
		\notag
		{\sf PowderHandlingDepositionSystem} \phantom{\ \equiv \ } & \\
		\notag
		{\sf InducedDefect} \equiv \ & {\sf EquipmentInducedDefect} \ \sqcap \\
		\notag
		& \exists{\sf isInducedBy}.({\sf MaterialDepositionSystem} \ \sqcap \\
		\notag
		& \exists{\sf isAffectedBy}.({\sf ByproductMaterialEjectionInducedDefect} \ \sqcup \\
		& {\sf SuperelevatedEdgesGeometricDefect}))
\end{align}
%}
%
It might be noted that defects induced by the powder handling and deposition system ({\sf PowderHandlingDepositionSystemInducedDefect}) are not influenced by recoating system characteristics (e.g., the wear of the recoater). In fact, most of the time the recoating system is not the direct source of these defects \cite{kleszczynski2012error,foster2015optical}. Instead, they are generated by the linear motion of the recoater that propagates inhomogeneities present on the powder bed (due to, e.g., super-elevated edges and spatters) along its moving direction.




\paragraph{Feedstock material-induced defects}
Powder quality, i.e., powder morphology, directly influences the quality (geometrical accuracy, porosity, and microstructure) as well as the performances (fatigue life) of the component \cite{sames2016metallurgy,das2003physical,van2007complexity,niu1999instability}. Another important feature of the powder is its flowability (powder fluidity), which depends on the particle size. If the powder particles are too small or too big, a smooth layer deposition cannot be achieved, eventually even stopping the process. Moreover, uniform powder deposition, smooth deposited powder layer, and uniform spreading, affect surface quality \cite{malekipour2018common,seyda2012investigation}.
Based on the observations above, we define the class {\sf FeedstockMaterialInducedDefect} by means of the following axiom:
%
\begin{align}
\notag
{\sf FeedstockMaterialInducedDefect} \equiv \ & {\sf InducedDefect} \ \sqcap \\
& \exists{\sf isInducedBy}.({\sf PackingDensity} \sqcup {\sf PowderSizeDistribution})
\end{align}
%





\paragraph{Process-induced defects}
Process parameters (e.g., laser power, scan speed, and hatch distance) influence the energy density that is introduced into the powder bed domain \cite{khairallah2016laser}. The energy density has been demonstrated to control the melt pool morphology and the cooling rate, thus ultimately influencing material microstructure \cite{LIAN2019107672}, geometric accuracy \cite{yeung2018}, as well as the porosity of final components \cite{MIKULA2021109851}.
Therefore, we include in the \emph{MAM4DefectOnt} module the class {\sf ProcessInducedDefect}, together with the two subclasses {\sf ByproductsAndMaterialEjectionInducedDefect} and {\sf ParameterAndScanStartegyInducedDefect} defined as follows:
%
\begin{align}
\notag
	{\sf ProcessInducedDefect} \equiv \ & {\sf InducedDefect} \ \sqcap
	\notag
	 \exists {\sf isInducedBy}.
({\sf Process} \ \sqcup \\
%\notag
	& {\sf ProcessParameter}) \\
%	& ({\sf Phenomenon}) \\
%	& \exists {\sf participatesIn}.{\sf AdditiveManufacturingProcess})) \\
		{\sf ByproductMaterialEjectionInducedDefect} \equiv \ & {\sf InducedDefect} \sqcap \exists{\sf isInducedBy}.{\sf Ejection} \\
		\notag
		{\sf ParameterScanStrategyInducedDefect} \equiv \ & {\sf InducedDefect} \ \sqcap \\
		\notag
		& \exists{\sf isInducedBy}.({\sf HatchingDistance} \ \sqcup \\
		\notag
		& {\sf HeatSourcePower} \ \sqcup \\
		& {\sf LayerThickness} \sqcup {\sf ScanningSpeed})
\end{align}

















%
%\subsubsection*{Subclasses and properties}\label{sec:properties}
%\todo[inline]{\AM{working here}}
%The relations in the presented ontology module are limited to \texttt{isA} and sub-relations of \texttt{hasSource}. Based on the above overview of the main defects and defect sources occurring in MAM, we have designed the module relationship. As an example, we consider the \texttt{PorosityDefect} class as depicted in \ref{fig:porosityClass}. This class has three sub-classes and three axioms which link it with the \texttt{DefectSource} sub-classes. The three sub-classes are: \texttt{InternalPorosityDefect}, which is characterized by small regular pores (see \ref{subfig:smallPores}), \texttt{InterlayerPorosityDefect}, with large, amorphous (acicular) pores, and \texttt{SurfacePorosityDefect} (see \ref{subfig:largePores}), which includes all the pores which can be found on the external surface. The class \texttt{PorosityDefect} can have three source of defects, according with the considered literature: i) process source, ii) equipment sources, and iii) feedstock material sources. All these three different sources seems to be affect the three sub-classes of porosity defects, thus they all inherit form the main class the \texttt{hasSource} properties. Following a similar procedure we have constructed all the other classes and sub-classes of the module.
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.75\textwidth]{figures/PorosityDefectClass.png}
%	\caption{Graphical representation of the \texttt{PorosityDefect} class and its axioms in the module.}
%	\label{fig:porosityClass}	
%\end{figure}
%
%\section{DefectOnto Modules}\label{sec:modules}
%
%\begin{figure}[h!]
%	\centering
%	\includegraphics[width=\textwidth]{figures/DefectOnto.png}
%	\caption{Graphical representation of DefectOnto modularity.}
%	\label{fig:DefectOntomodules}	
%\end{figure}
%
%As described in Section~\ref{sec:state-of-the-art}, a few ontologies have been proposed in recent years for additive manufacturing. These ontologies are very different form each other, thus making almost impossible to define a module -- such as the MAM defects ontology module presented in Section~\ref{sec:AM-defect-module} -- which is at the same time general and fully merged with the specific AM ontology. Therefore, we have tried to formulate the defect module as a standalone set of classes and axioms which we then aim at AMmodule with the axioms and classes of specific AM ontologies.
%%
%\todo[inline]{\MC{Questi paragrafi sono ancora necessari??}}
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	\item DefectCharacteristic
%DefectSource
%DesignSource
%OrientationSource
%SupportSource
%EquipmentSource
%BaseplateSource
%BeamScanningDeflectionSystemSource
%BuildChamberEnvironmentalControlSource
%PowderHandlingDepositionSystemSource
%FeedstockMaterialSource
%ProcessSource
%ByproductsAndMaterialEjectionSource
%ParameterAndScanStrategySource
%Defect
%BallingDefect
%CrackingDelaminationDefect
%GeometricDefect
%MicrostructuralDefect
%PorosityDefect
%SurfaceDefect
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	\item hasDesignSource
%hasSource
%hasProcessSource
%hasFeedstockMaterialSource
%hasEquipmentSource
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item hasBeamRadius
%\end{itemize}

==> ArXiv/main/sec_ontomodule_am_defectcore_typesource.tex <==
\subsubsection{Relating defects types and sources in \emph{MAM4DefectOnt}}
\label{sec:bridgeaxioms}

\noindent
Following~\citet{grasso2017process}, Table~1 (and references therein), in this section we discuss the mappings connecting each type of MAM defects formalised in Section~\ref{sec:defecttype} with the corresponding causes identified in the literature, and modelled in terms of {\sf InducedDefect} subclasses in Section~\ref{sec:defectsource}.
Such mappings consist of subsumption axioms of the form
%\begin{enumerate*}[label=(\arabic*)]
%\item
%\label{item:axiompositive}
$A \sqsubseteq C$
%and
%\item\label{item:axiomnegative} $A \sqsubseteq \lnot C'$,
%\end{enumerate*}
where: $A$ is any of the classes {\sf BallingDefect}, {\sf CrackingDefect}, {\sf GeometricDefect}, {\sf MicrostructuralDefect}, {\sf PorosityDefect}, {\sf SourfaceRoughnessDefect}; and $C$ is the union of subclasses of {\sf InducedDefect}.
These axioms
%Axioms of the form~\ref{item:axiompositive}
express the fact that defects of type $A$ are
documented
%considered
in the literature to be caused by at least one of the MAM features that characterise some disjoints in $C$.
%Axioms of the form~\ref{item:axiomnegative}, instead, capture the information that defects of type $A$ are considered not to be caused by any of the MAM features characterising a disjoint in $C'$.

For instance, it is
documented in
%known from
the literature~\cite{grasso2017process} that porosity defects can be induced by:
the beam scanning or deflection system;
the build chamber environmental control;
the powder handling and deposition system;
the process parameters and scan strategies;
byproducts and material ejections.
%On the other hand, porosity defects are known to be not influenced by the following MAM features: baseplate properties; supports characteristics; and part orientation.
Accordingly, we express in \emph{MAM4DefectOnt} that the class {\sf PorosityDefect} is included in the union of
the following classes:
{\sf BeamScanningDeflectionSysemInducedDefect},
{\sf BuildChamberEnvironmentalControlInducedDefect},
{\sf PowderHandlingDepositionSystemInducedDefect},
{\sf ParameterScanStrategyInducedDefect},
{\sf ByproductMaterialEjectionInducedDefect},
and
{\sf FeedstockMaterialInducedDefect}.
%whereas it is disjoint from the union of {\sf BaseplateInducedDefect}, {\sf SupportInducedDefect}, and {\sf OrientationInducedDefect}.
%We present in the following a complete list of such axioms.
%%A complete list of these axioms is provided in the Appendix.

In the rest of this section, we list the mappings axioms for each of the subclasses of {\sf Defect} discussed in Section~\ref{sec:defecttype}.

\paragraph{Balling defect sources}


\begin{align}
		\notag
	{\sf BallingDefect} \sqsubseteq \ & {\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		& {\sf OrientationInducedDefect}
\end{align}


%\begin{align}
%		\notag
%	{\sf BallingDefect} \sqsubseteq
%	\lnot ( &
%	{\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf BaseplateInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf ByproductMaterialEjectionInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf SupportInducedDefect} \ \sqcup \\
%		& {\sf FeedstockMaterialInducedDefect})
%\end{align}


\paragraph{Cracking and delamination defect sources}


\begin{align}
		\notag
	{\sf CrackingDefect} \sqsubseteq \ & {\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
		\notag
		& {\sf BaseplateInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		& {\sf SupportInducedDefect}
\end{align}

%\begin{align}
%		\notag
%	{\sf CrackingDefect} \sqsubseteq
%	\lnot ( &
%	{\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf ByproductMaterialEjectionInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf OrientationInducedDefect} \ \sqcup \\
%		& {\sf FeedstockMaterialInducedDefect})
%\end{align}





\paragraph{Geometric defect sources}

\begin{align}
		\notag
	{\sf GeometricDefect} \sqsubseteq \ & {\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf BaseplateInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		\notag
		& {\sf SupportInducedDefect} \ \sqcup \\
		\notag
		& {\sf OrientationInducedDefect} \ \sqcup \\
		& {\sf FeedstockMaterialInducedDefect}
\end{align}

%\begin{align}
%		\notag
%	{\sf GeometricDefect} \sqsubseteq
%	\lnot ( &
%	{\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
%		& {\sf ByproductMaterialEjectionInducedDefect})
%\end{align}





\paragraph{Microstructural defect sources}


\begin{align}
		\notag
	{\sf MicrostructuralDefect} \sqsubseteq \ & {\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
			\notag
		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		\notag
		& {\sf ByproductMaterialEjectionInducedDefect} \ \sqcup \\
		\notag
		& {\sf OrientationInducedDefect} \ \sqcup \\
		& {\sf FeedstockMaterialInducedDefect}
\end{align}


%\begin{align}
%		\notag
%	{\sf MicrostructuralDefect} \sqsubseteq
%	\lnot ( &
%	{\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf BaseplateInducedDefect} \ \sqcup \\
%		& {\sf SupportInducedDefect})
%\end{align}



\paragraph{Porosity defect sources}


\begin{align}
		\notag
	{\sf PorosityDefect} \sqsubseteq \ & {\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
		\notag
		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		\notag
		& {\sf ByproductMaterialEjectionInducedDefect} \ \sqcup \\
		& {\sf FeedstockMaterialInducedDefect}
\end{align}


%\begin{align}
%		\notag
%	{\sf PorosityDefect} \sqsubseteq
%	\lnot (
%		& {\sf BaseplateInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf SupportInducedDefect} \ \sqcup \\
%		& {\sf OrientationInducedDefect})
%\end{align}






\paragraph{Surface roughness defect sources}



\begin{align}
		\notag
	{\sf SurfaceRoughnessDefect} \sqsubseteq \ 
		& {\sf PowderHandlingDepositionSystemInducedDefect} \ \sqcup \\
		\notag
		& {\sf ParameterScanStrategyInducedDefect} \ \sqcup \\
		\notag
		& {\sf SupportInducedDefect} \ \sqcup \\
		\notag
		& {\sf OrientationInducedDefect} \ \sqcup \\
		& {\sf FeedstockMaterialInducedDefect}
\end{align}



%\begin{align}
%		\notag
%	{\sf SurfaceRoughnessDefect} \sqsubseteq
%	\lnot (
%		& {\sf BeamScanningDeflectionSystemInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf BuildChamberEnvironmentalControlInducedDefect} \ \sqcup \\
%		\notag
%		& {\sf BaseplateInducedDefect} \ \sqcup \\
%		& {\sf ByproductMaterialEjectionInducedDefect})
%\end{align}

\subsubsection{Competency questions for \emph{MAM4DefectOnt}}
\label{sec:CQsMAM4DefectOnt}
\noindent
The \emph{MAM4DefectOnt} module, together with its \emph{Spatial4DefectOnt} submodule, allow us to answer, for instance, to the following CQs:
%
%			\begin{itemize}[leftmargin=0cm]
				%
%				\item[CQAm] MAM-related CQs
				\begin{enumerate}[label={CQAm.\arabic*}, leftmargin=*]
%					\item[CQAm.1] Is the feature ${\sf d}$ an instance of a defect?
					\item[CQAm.2] Is the feature ${\sf d}$ an instance of a porosity defect?
%					\item[CQAm.3] Which type of defect is defect ${\sf d}$?
%					\item[CQAm.4] By which parameters can defect ${\sf d}$ be influenced?
%					\item Is defect ${\sf d}$ induced by a process parameter?
				\end{enumerate}
%				\item[CQSp] Spatial-related CQs
				\begin{enumerate}[label={CQSp.\arabic*}, leftmargin=*]
%					\item Is the MAM product {\sf p} affected by any equipment-induced surface defects?
%					\item Are there balling defects located on the surface layers of product {\sf p}?
%					\item[CQSp.1] Is there an instance of a balling defect overlapping with a surface layer?
					\item[CQSp.2] What is the length in metres of the cracking defect instance {\sf d}?
%					\item[CQSp.3] \ldots
%%					\item[CQSp.3] What is the volume of the bounding box {\sf b} for balling defect {\sf d}?
%%					\item[CQSp.3] What is the dimension of {\sf d}?
%%					\item[CQSp.1] Where is located the defect in the component?
%%					\item[CQSp.2] What is the morphology of the defect?
%%					\item[CQSp.3] What is the size of the defect?
				\end{enumerate}
%			\end{itemize}
		


%\todo[inline]{\AM{todo add axioms connecting types of defects and possible sources}}


==> ArXiv/main/sec_ontomodule_am_others.tex <==
%\subsubsection{\textnormal{\emph{nist4defectont}}}
%The sub-module {\emph{nist4defectont}} inherit classes and properties from the NIST AM ontology, an OWL ontology of concepts of additive manufacturing produced as part of NIST's Systems Integration for Additive Manufacturing project \footnote{https://www.nist.gov/programs-projects/systems-integration-additive-manufacturing}. Such an ontology is organised into three packages: AMProcessOntology, ModelOntology, and AMOntology. In the present work we take axioms and properties mainly from the first set of entities since they are intended to provide knowledge about the AM process, with a special focus on MAM processes. 
%
%%%
%%\paragraph{Main Classes}
%%%
%%\begin{itemize}
%%	\item PowderBedFusionProcess
%%ElectronBeamMelting
%%Material
%%ProcessCharacteristic
%%CrystallineMaterial
%%ResidualStressDistribution
%%SelectiveLaserMelting
%%MetallicCrystalline
%%SemiCrystallineThermoplastic
%%Shrinkage
%%AmorphousThermoplastic
%%Abstract
%%MetalAlloy
%%MaterialVendorSpecification
%%Microstructure
%%Ceramic
%%MeltPoolTemperature
%%Physical
%%SelectiveLaserSintering
%%AdditiveManufacturingProcess
%%AmorphousMaterial
%%Characteristic
%%DentriticGrainSize
%%ProcessSignature
%%EquipmentParameter
%%HardMetal
%%Void
%%ProcessParameter
%%HeatSourcePower
%%DirectMetalLaserSintering
%%DirectMetalLaserMelting
%%HatchingDistance
%%LayerThickness
%%MeltPoolSignature
%%PowderBedFusionProcessParameter
%%DendriteGrainOrientation
%%MeltPoolShape
%%ScanningSpeed
%%\end{itemize}
%%%
%%\paragraph{Main Properties}
%%%
%%\begin{itemize}
%%	\item appliesTo
%%functionOf
%%hasCharacteristic
%%influencedBy
%%influences
%%partOf
%%providedBy
%%provides
%%\end{itemize}
%%%
%%\paragraph{Main Data Properties}
%%%
%%\begin{itemize}
%%	\item hasBeamRadius
%%hasScanningSpeed
%%hasValue
%%\end{itemize}
%%
%\subsubsection{\textnormal{\emph{mason4defectont}}}
%This sub-module inherits classes and properties from the MASON ontology and it is intended to provide geometric knowledge on defects as well as on the component.
%%%
%%\paragraph{Main Classes}
%%%
%%\begin{itemize}
%%	\item Entity
%%Geometric\_entity
%%Shape
%%Symmetry
%%Topology
%%Geometric\_entity\_for\_manufacturing
%%Linear\_entity
%%Revolution\_entity
%%Geometric\_flaw
%%Entity\_geometric\_flaw
%%Geometric\_flaw\_1st\_order
%%Geometric\_flaw\_2nd\_order
%%Geometric\_flaw\_3rd\_order
%%Geometric\_flaw\_4th\_order
%%Geometric\_flaw\_between\_entities
%%Raw\_material
%%Alloy
%%Aluminium
%%Glass
%%Plastic
%%Steel
%%Wood
%%\end{itemize}
%%%
%%\paragraph{Main Properties}
%%%
%%\begin{itemize}
%%	\item hasShape
%%hasSymmetry
%%isMadeOf
%%ofTopology
%%\end{itemize}
%%%
%%\paragraph{Main Data Properties}
%%%
%%\begin{itemize}
%%	\item corrugation
%%rugosity
%%\end{itemize}
%%%
%\subsubsection{\textnormal{\emph{onto4add4defectont}}}
%%
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	\item PhysicalObject
%Material
%AMSupportStructure
%AMLayer
%Gas
%Process
%MfgProcess
%AMProcess
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	\item hasPart
%hasInput
%hasMaterialState
%hasMechanism
%hasParticipant
%hasSubprocess
%inputOf
%madeOf
%makes
%materialStateOf
%occursIn
%outputOf
%participatesIn
%realisedBy
%time:after
%time:before
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item hasBuildDurationInMinutes
%hasBuildingCostInEuro
%hasDurationInMinutes
%hasFinishTimeValue
%hasStartTimeValue
%hasTemperatureInCelsius
%hasTemperatureInCelsiusDuringFabrication
%\end{itemize}
%
%In this work we present, as an example, the AMmodule procedure that we have done to integrate the MAM defects ontology module into the AM ontology proposed by the National Institute of Standards and Technology (NIST) in \cite{lu2015towards}, this OWL ontology can be found in an open repository at \href{https://github.com/iassouroko/AMontology}{https://github.com/iassouroko/AMontology}. Such an ontology is organized into two main classes: \texttt{Abstract} and \texttt{Physical}. Accordingly, when AMmodule our module into this framework, we have decided to insert \texttt{DefectSource} as sublcalss of the former and \texttt{Defect} as subclass of the latter. Herein, we limit to describe the main axioms and properties we have used during the AMmodule procedure.  
%%
%
%
%%\subsection{NIST classes and properties}\label{ssec:axiomsMerge}
%
%In the following, we describe the axioms used to integrate the classes of the proposed ontology module into the NIST AM ontology. 
%%
%\paragraph{InfluencedBy}
%This is the axioms present in the NIST ontology we have more extensively used to integrate our module. In fact, each defect has one or more sources but it is also influenced by some characteristics of the process. In particular, each defect can influenced by the so-called process signature (e.g., melt pool shape and temperature, microstructure, residual stresses), that are quantifiable characteristic of the specific MAM process s well as by the process parameters. Therefore, as depicted in \ref{fig:mainclassesMerged}, the main class \texttt{Defect} is connected by means of the \texttt{InfluencedBy} axioms to the \texttt{Characteristic} class of the AM ontology, which includes as a subclasses \texttt{ProcessSignature} and \texttt{ProcessParameters}.
%%
%%\begin{figure}[h!]
%%	\centering
%%	\includegraphics[width=0.66\textwidth]{figures/MainClassesMerged.png}
%%	\caption{Graphical representation of the ontology module main classes.}
%%	\label{fig:mainclassesMerged}	
%%\end{figure}
%%
%%\paragraph{hasCharacteristic}
%%The other key axiom we employed to merge the module into AM ontology is  \texttt{hasCharacteristic}. As depicted in \ref{fig:mainclassesMerged}, we have used this axiom to link each defect source of our module with a subclass of the AM ontology \texttt{Characteristic} class. The scope is to associate a measurable entity, i.e., a characteristic, of the process to each defect source. 

==> ArXiv/main/sec_ontomodule_measure.tex <==
\subsection{\emph{Measure4DefectOnt} Module}
\label{sec:meas-mod}

\noindent
This module is intended to provide axioms, classes, and properties that are necessary to describe AM process and product features requiring notions related to measures, measuring units, and scales. Relevant classes (e.g., {\sf Temperature}, {\sf CelsiusTemperature}, {\sf Area}, {\sf Length}) are included in its only submodule, \emph{OM4ExtruOnt}, which is  imported from the \emph{ExtruOnt}~\cite{RamEtAl20} by leveraging the modular structures of both \emph{ExtruOnt} and \emph{DefectOnt} ontologies. 
\citeauthor{RamEtAl20} obtain this submodule from the OM ontology via a pruning process that retains only those concepts and properties pertaining to manufacturing process and components.
%In such a submodule, the concepts that are useful to describe manufacturing process and components have been already selected from the OM ontology.
In particular, this module is intended to provide the necessary knowledge to address, for instance, the following competency question:
%
%\todo[inline]{\AM{todo add CQs from ORSD}}
\begin{enumerate}[label={CQMe.\arabic*}, leftmargin=*]
%	\item What is the melt pool temperature in degrees Celsius?
%	\item What is the thickness in millimetres of layer {\sf l}?
	\item[CQMe.3] What is the length in meters of the cracking defect instance {\sf d}?
\end{enumerate}
%
%%
%\subsubsection{\textnormal{\emph{OMExtruOnt4DefectOnt}}}
%%
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	 \item Dimension
%Measure
%Prefix
%SIPrefix
%Quantity
%AmountOfMoney
%Cost
%AngularSpeed
%AngularVelocity
%Area
%Capacitance
%DynamicViscosity
%ElectricalResistance
%ElectricCurrent
%ElectricPotential
%Frequency
%Length
%Depth
%Diameter
%Distance
%Height
%Thickness
%Width
%Mass
%BodyMass
%Number
%Power
%Pressure
%Ratio
%Speed
%Velocity
%Stress
%CompressiveStress
%Temperature
%CelsiusTemperature
%FahrenheitTemperature
%ThermalConductivity
%ThermalResistance
%Time
%Date
%Duration
%Period
%Torque
%Volume
%VolumetricFlowRate
%Wavenumber
%Scale
%CelsiusTemperatureScale
%FahrenheitTemperatureScale
%IntervalScale
%RatioScale
%Temperature\_scale
%ThermodynamicTemperatureScale
%SystemOfUnits
%Unit
%AmountOfMoneyUnit
%AngularSpeedUnit
%AreaUnit
%CapacitanceUnit
%CompoundUnit
%DynamicViscosityUnit
%ElectricalResistanceUnit
%ElectricCurrentUnit
%ElectricPotentialUnit
%FrequencyUnit
%LengthUnit
%MassUnit
%NumberUnit
%PowerUnit
%PrefixedUnit
%PrefixedAmpere
%PrefixedAre
%PrefixedDegreeCelsius
%PrefixedFarad
%PrefixedGram
%PrefixedHertz
%PrefixedKelvin
%PrefixedLitre
%PrefixedMetre
%PrefixedOhm
%PrefixedPascal
%PrefixedSecond-Time
%PrefixedTonne
%PrefixedUnifiedAtomicMassUnit
%PrefixedVolt
%PrefixedWatt
%PressureUnit
%RatioUnit
%SingularUnit
%SpeedUnit
%StressUnit
%TemperatureUnit
%CelsiusTemperatureUnit
%FahrenheitTemperatureUnit
%ThermalConductivityUnit
%ThermalResistanceUnit
%TimeUnit
%TorqueUnit
%VolumetricFlowRateUnit
%VolumeUnit
%WavenumberUnit
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	  \item commonlyHasUnit
%hasBase
%hasBaseQuantity
%hasBaseUnit
%hasDenominator
%hasDerivedQuantity
%hasDerivedUnit
%hasDimension
%hasNumerator
%hasPhenomenon
%hasPrefix
%hasQuantity
%hasScale
%hasTerm1
%hasTerm2
%hasUnit
%hasValue
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item hasExponent
%hasFactor
%hasNumericalValue
%hasOff-Set
%hasSIAmountOfSubstanceDimensionExponent
%hasSIElectricCurrentDimensionExponent
%hasSILengthDimensionExponent
%hasSILuminousIntensityDimensionExponent
%hasSIMassDimensionExponent
%hasSIThermodynamicTemperatureDimensionExponent
%hasSITimeDimensionExponent
%\end{itemize}

==> ArXiv/main/sec_ontomodule_sensor.tex <==
%
\subsection{\emph{Sensor4DefectOnt} Module}
\label{sec:sens-mod}
%
This module is intended to enable domain experts and/or online defect detection systems to gain insights from data measured by means of sensors installed on the AM machine. In particular, the axioms of the class {\sf FeatureOfInterest} together with its related properties and subclasses are present in this module through the submodule of the SSN ontology, \emph{SSN4DefectOnt} .
Moreover, this module provides useful concepts to evaluate the quality of MAM processes allowing to potentially perform online defect diagnosis and troubleshooting. In particular, \emph{sensor4DefectOnt} allows to answer the following competency questions:
\begin{enumerate}[label={CQSe.\arabic*}, leftmargin=*]
%					\item Which sensors are hosted by platform {\sf pl}?
					\item[CQSe.2] Does any sensor hosted by platform {\sf pl} observe an instance of a porosity defect?
\end{enumerate}
 
%\subsubsection{\textnormal{\emph{ssn4defectont}}}
%%
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	 \item FeatureOfInterest
%Observation
%Sample
%ObservableCharacteristic
%Platform
%Property
%Result
%Sampling
%Stimulus
%System
%Sensor
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	  \item detects
%hasFeatureOfInterest
%hasProperty
%hasResult
%hasResultingSample
%hosts
%isHostedBy
%isPropertyOf
%madeBySensor
%observedProperty
%observes
%phenomenonTime
%qualityOfObservation
%wasOriginatedBy
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item hasSimpleResult
%resultTime
%\end{itemize}
%%

==> ArXiv/main/sec_ontomodule_spatial.tex <==
\subsection{\emph{Spatial4DefectOnt} Module}
\label{sec:spat-mod}
The \emph{Spatial4DefectOnt} is composed by two submodules: \emph{geosparql4defectont} and \emph{mason4defectont}. The former is derived from the GEOSPARQL ontology taking into account a set of axioms useful to describe spatial features of MAM defects, whereas the latter is derived from the MASON ontology and it is a submodule also of the \emph{MAM4DefectOnt} module (see \cref{sec:AM-mod}). In fact, the modular approach followed in the present work and described in \cref{sec:ont-design-meth} allows to take specific axioms form a third-part ontology (e.g., MASON), re-using in diffent modules the same submodule (e.g., \emph{mason4defectont}). The \emph{Spatial4DefectOnt} module is intended to answer the following competency questions:

%\subsubsection{\textnormal{\emph{geosparql4defectont}}}
%%
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	\item SpatialObject
%Feature
%Geometry
%SpatialObjectCollection
%FeatureCollection
%GeometryCollection
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	\item ehInside
%	  hasPerimeterLength
%	  hasLength
%	  hasDefaultGeometry
%	  hasGeometry
%	  ehCoveredBy
%	  ehOverlap
%	  hasVolume
%	  hasCentroid
%	  ehCovers
%	  ehContains
%	  hasBoundingBox
%	  hasSpatialResolution
%	  ehEquals
%	  defaultGeometry
%	  hasArea
%	  ehDisjoint
%	  ehMeet
%	  hasSize
%	  hasSpatialAccuracy
%	  sfContains
%	  sfCrosses
%	  sfDisjoint
%	  sfEquals
%	  sfIntersects
%	  sfTouches
%	  sfOverlaps
%	  sfWithin
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item coordinateDimension
%	  dimension
%	  hasMetricArea
%	  hasMetricLength
%	  hasMetricPerimeterLength
%	  hasMetricSize
%	  hasMetricSpatialAccuracy
%	  hasMetricSpatialResolution
%	  hasMetricVolume
%	  hasSerialization
%	  isEmpty
%	  isSimple
%	  spatialDimension
%\end{itemize}
%%
%%\subsection{All Ontologies}
%%
%%
%%
%%\subsubsection{NIST}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Abstract
%%	\item Physical
%%	\item Characteristic
%%	\item ProcessParameter ($+$ subclasses)
%%	\item ProcessSignature ($+$ subclasses)
%%	\item Material ($+$ subclasses)
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasCharacteristic
%%	\item influencedBy
%%	\item influences
%%\end{itemize}
%%
%%
%%
%%\subsubsection{MASON}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Manufacturing\\_concept
%%\end{itemize}
%%
%%
%%\subsubsection{PartOf}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasPart
%%	\item isPartOf
%%\end{itemize}
%%
%%
%%\subsubsection{EMMO}
%%
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Observer
%%	\item MeasuringInstrument
%%	\item MeasuringSystem
%%\end{itemize}
%%
%%
%%
%%
%%\subsubsection{Onto4Additive}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item PhysicalObject ($\equiv$ SpatialObject) (remove? also in others?)
%%	\item Process
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item typeOf
%%	\item hasParticipant
%%	\item hasSubprocess
%%	\item participatesIn
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasBuildDurationInMinutes
%%	\item hasBuildSpeedInMillimetrePerSecond
%%	\item hasDurationInMinutes
%%	\item hasFeedRateInKilogramPerHour
%%	\item hasFinishTimeValue
%%	\item hasStartTimeValue
%%\end{itemize}
%%
%%
%%
%%\subsubsection{SAREF}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item FeatureOfInterest
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item makesMeasurement ($\equiv$ measures)
%%	\item measurementMadeBy ($\equiv$ isMeasuredBy)
%%\end{itemize}
%%
%%
%%\subsubsection{SSN/SOSA}
%%
%%\begin{itemize}
%%	\item Property ($\equiv$ Characteristic)
%%	\item ObservableProperty
%%	\item Sensor
%%	\item Platform
%%	\item Stimulus
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item detects
%%	\item hosts
%%	\item isHostedBy
%%	\item observes
%%	\item isObservedBy
%%\end{itemize}
%%
%%
%%
%%\subsubsection{GeoSPARQL}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item SpatialObject ($\equiv$ PhysicalObject)
%%	\item Feature
%%	\item Geometry
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasDefaultGeometry
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasMetricArea
%%	\item hasMetricLength
%%	\item hasMetricPerimeterLength
%%	\item hasMetricSize
%%	\item hasMetricVolume
%%\end{itemize}
%%
%%
%%
%%
%%\subsubsection{OM Ontology}
%%
%%\paragraph{Classes}
%%
%%\begin{itemize}
%%	\item Measure
%%	\item Unit
%%	\item hasUnit
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasNumericalValue
%%\end{itemize}
%%
%%
%%
%%\subsection{Our Signature}
%%
%%
%%\paragraph{Classes}
%%
%%\begin{itemize}
%%	\item DefectCharacteristic
%%	\item DefectSource ($+$ subclasses)
%%	\item Defect ($+$ subclasses)
%%	\item MetrologicalCharacteristic (find substitute?)
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasMeasure (change? remove? find OM substitute?)
%%	\item isMeasureOf (change? remove? find OM substitute?)
%%	\item measures (find SOSA substitute?)
%%	\item isMeasuredBy (find SOSA substitute?)
%%	\item hasSource ($+$ subproperties)
%%	\item isSourceOf
%%\end{itemize}
%%
%%
%%\paragraph{Properties}

==> ArXiv/main/sec_relwork.tex <==
\section{Related work}\label{sec:state-of-the-art}

\subsection{MAM-related literature}

%Transforming measured data into useful information and knowledge to detect the causality links and the complex process-structure-property relationships in manufacturing processes is one of the main issues in AM research \cite{debroy2018additive}. At industrial level, Powder Bed Fusion (PBF) MAM is nowadays the most widespread technology due to its capability to deliver parts with high surface quality and remarkable mechanical properties. PBF process is a layer-by-layer process, where a layer of metal powder is spread by means of a roller on top of a build plate and metal powder particles are selectively melted by means of a localized moving laser heat source \cite{frazier2014metal}. The localized nature of the resulting melt pool induces rapid melting-solidification cycles that are responsible for part deflections and residual stresses \cite{Bartlett2019}. Moreover, due to is multi-scale and multi-physics nature, physical phenomena involved in PBF processes are difficult to control. Such an issue can lead to process-induced material discontinuities e.g., lack-of-fusion and keyhole porosity, balling, crack and delamination \cite{DUPLESSIS2020108385}. Moreover, the overall process is characterized by complex and not yet fully understood relationships among material microstructure, part geometry, process parameters, and mechanical properties and performances \cite{smith2016linking}. Even if process-induced defects play a key role influencing part properties and performances (e.g., elastic and elastoplastic behavior, ultimate tensile stress, and fatigue life) a rigorous and formal knowledge-based representation of MAM defects is not yet available in the literature. 

\noindent
\citet{malekipour2018common}  identify, analyze, and classify the most common defects in PBF MAM, defining the relationships among defects and their contributing parameters. To develop a suitable online monitoring control strategy, defects are organized into categories based on their manufacturing features and control purposes.
\citet{kyogoku2020review} review the literature regarding defect generation mechanisms in PBF processes and their mitigation strategies. 
\citet{snow2020invited} outline the state-of-the-art knowledge of gas porosity and lack-of-fusion flaws due to melt pool instabilities in PBF processes.
\citet{grasso2017process} present a defect classification of PBF process-induced defects based on process signatures, to support in-situ monitoring and online defect detection.
The present contribution follows defects taxonomies proposed in \cite{grasso2017process} (and references therein), integrating it with other literature resources (of both non-ontological and ontological nature).
%and translating this knowledge into formal ontology axioms.
%All the above mentioned review articles introduce MAM defects classifications and taxonomies. However, they do not provide any ontology for AM defects, i.e., the relationships among defects and process signatures, generation mechanisms, and corresponding mitigation strategies are not yet formalized in a way allowing to perform high-level reasoning to inherit from data the complex process-structure-property relationships occurring in MAM.


%
\subsection{Ontology-related literature}
%\todo[inline]{\AM{todo add ontology-related refs.}}
\noindent
Given its closely related focus (despite not overlapping with ours,  content-wise), we relied on \emph{ExtruOnt}, an ontology for the description of an extruder components proposed by~\citet{RamEtAl20}, as a gold standard for the development of our knowledge base, adhering to the authors' methodological, design, and presentation choices. 
%

With a broader scope, other upper or domain ontologies for AM have been proposed in the literature.
The Manufacturing's Semantics Ontology (MASON)~\cite{LemEtAl06} is an upper ontology for the conceptualisation of core additive manufacturing domain notions.
%A Proposal For An Ontology Of Manufacturing Domain
The US~National Institute of Standards and Technology (NIST) propose an ontology for AM, that we label NIST AM~\cite{WitEtAl14,WitEtAl16}, to support the development of laser and thermal metamodels.
%ONTOLOGY-BASED LASER AND THERMAL METAMODELS FOR METAL-BASED ADDITIVE MANUFACTURING
%Toward Metamodels for Composable and Reusable Additive Manufacturing Process Models
%
Towards interoperable knowledge and data management in applications, \citet{SanEtAl19} introduce another ontology for AM (Onto4Additive), based on the upper Descriptive Ontology for Linguistic and Cognitive Engineering (DOLCE)~\cite{BorMas09}.
%Borgo, S., and Masolo, C. Foundational choices in DOLCE
%

Other related AM ontologies include the following (cf. also literature reviews in~\citet{SanEtAl19} and~\citet{RamEtAl20}):
the Additive Manufacturing Ontology (AMO)~\cite{AliEtAl19},
%A product life cycle ontology for additive manufacturing
based on the upper Basic Formal Ontology (BFO)~\cite{arp2015building};
%Arp, Smith Building ontologies with basic formal ontology.;
the Innovative Capabilities of Additive Manufacturing
(ICAM) ontology~\cite{HagEtAl18};
%A Knowledge-Based Method for Innovative Design for Additive Manufacturing Supported by Modular Ontologies
%Mahmoud Dinar, David W. Rosen, A Design for Additive Manufacturing Ontology
%as well as the already mentioned NIST AM ontology.
%
%L.M. Daniele, M. Punter, C. Brewster, R. García Castro, M. Poveda and A. Fernández, A SAREF Extension for Se- mantic Interoperability in the Industry and Manufacturing Domain, in: Enterprise Interoperability, John Wiley & Sons, Ltd, 2018, pp. 201?207, Chapter 25. ISBN 9781119564034. doi:10.1002/9781119564034.ch25
a Smart Applications Reference (SAREF)~\cite{appliances2017smartm2m}
%ETSI, SmartM2M; Smart Applicances; Reference Ontology and oneM2M Mapping, Technical specification, TS 103 264 V2.1.1, ETSI, 2017.
extension for semantic interoperability in the industry and manufacturing domain (SAREF4INMA)~\cite{DanEtAl18};
%L.M. Daniele, M. Punter, C. Brewster, R. García Castro, M. Poveda and A. Fernández, A SAREF Extension for Se- mantic Interoperability in the Industry and Manufacturing Domain, in: Enterprise Interoperability
the Semantically Integrated Manufacturing Planning Model (SIMPM)~\cite{vsormaz2019simpm};
%An Upper-level ontology for manufacturing process plan network genera- 23 tion
the Manufacturing Resource Capability Ontology (MaRCO)~\cite{JarEtAl19};
%E. Järvenpää, N. Siltala, O. Hylli and M. Lanz, The development of an ontology for describing the capabilities of manufacturing resources
the Manufacturing Service Description Language (MSDL) ontology~\cite{ameri2006upper};
%F. Ameri and D. Dutta, An upper ontology for manufacturing service description
the
Politecnico di Milano--Production Systems Ontology (P-PSO) ~\cite{garetti2012p};
%M. Garetti and L. Fumagalli, P-PSO ontology for manufactur- ing systems
the
Ontology of Standard for the Exchange of Product model data (OntoSTEP)~\cite{BarEtAl12};
%R. Barbau, S. Krima, R. Sudarsan, A. Narayanan, X. Fiorentini, S. Foufou and R.D. Sriram, OntoSTEP: Enriching product model data using ontologies
the ontologies proposed by~\citet{DinRos17},~\citet{liang2018ontology},~\citet{roh2021ontology}, and~\citet{li2022description}.
%Liang, J. S. An ontology-oriented knowledge methodology for process planning in additive layer manufacturing
%
Finally, within the EU-funded project EMMC, the recently proposed European Materials Modelling Ontology (EMMO)~\cite{HorEtAl20} provides a standard representational upper (nominalistic) ontology framework based on state-of-the-art knowledge on material modelling and engineering.





==> sec_ontomodule_spatial.tex <==
\subsection{\emph{Spatial4DefectOnt} Module}
\label{sec:spat-mod}
The \emph{Spatial4DefectOnt} is composed by two submodules: \emph{geosparql4defectont} and \emph{mason4defectont}. The former is derived from the GEOSPARQL ontology taking into account a set of axioms useful to describe spatial features of MAM defects, whereas the latter is derived from the MASON ontology and it is a submodule also of the \emph{MAM4DefectOnt} module (see \cref{sec:AM-mod}). In fact, the modular approach followed in the present work and described in \cref{sec:ont-design-meth} allows to take specific axioms form a third-part ontology (e.g., MASON), re-using in diffent modules the same submodule (e.g., \emph{mason4defectont}). The \emph{Spatial4DefectOnt} module is intended to answer the following competency questions:

%\subsubsection{\textnormal{\emph{geosparql4defectont}}}
%%
%\paragraph{Main Classes}
%%
%\begin{itemize}
%	\item SpatialObject
%Feature
%Geometry
%SpatialObjectCollection
%FeatureCollection
%GeometryCollection
%\end{itemize}
%%
%\paragraph{Main Properties}
%%
%\begin{itemize}
%	\item ehInside
%	  hasPerimeterLength
%	  hasLength
%	  hasDefaultGeometry
%	  hasGeometry
%	  ehCoveredBy
%	  ehOverlap
%	  hasVolume
%	  hasCentroid
%	  ehCovers
%	  ehContains
%	  hasBoundingBox
%	  hasSpatialResolution
%	  ehEquals
%	  defaultGeometry
%	  hasArea
%	  ehDisjoint
%	  ehMeet
%	  hasSize
%	  hasSpatialAccuracy
%	  sfContains
%	  sfCrosses
%	  sfDisjoint
%	  sfEquals
%	  sfIntersects
%	  sfTouches
%	  sfOverlaps
%	  sfWithin
%\end{itemize}
%%
%\paragraph{Main Data Properties}
%%
%\begin{itemize}
%	\item coordinateDimension
%	  dimension
%	  hasMetricArea
%	  hasMetricLength
%	  hasMetricPerimeterLength
%	  hasMetricSize
%	  hasMetricSpatialAccuracy
%	  hasMetricSpatialResolution
%	  hasMetricVolume
%	  hasSerialization
%	  isEmpty
%	  isSimple
%	  spatialDimension
%\end{itemize}
%%
%%\subsection{All Ontologies}
%%
%%
%%
%%\subsubsection{NIST}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Abstract
%%	\item Physical
%%	\item Characteristic
%%	\item ProcessParameter ($+$ subclasses)
%%	\item ProcessSignature ($+$ subclasses)
%%	\item Material ($+$ subclasses)
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasCharacteristic
%%	\item influencedBy
%%	\item influences
%%\end{itemize}
%%
%%
%%
%%\subsubsection{MASON}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Manufacturing\\_concept
%%\end{itemize}
%%
%%
%%\subsubsection{PartOf}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasPart
%%	\item isPartOf
%%\end{itemize}
%%
%%
%%\subsubsection{EMMO}
%%
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item Observer
%%	\item MeasuringInstrument
%%	\item MeasuringSystem
%%\end{itemize}
%%
%%
%%
%%
%%\subsubsection{Onto4Additive}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item PhysicalObject ($\equiv$ SpatialObject) (remove? also in others?)
%%	\item Process
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item typeOf
%%	\item hasParticipant
%%	\item hasSubprocess
%%	\item participatesIn
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasBuildDurationInMinutes
%%	\item hasBuildSpeedInMillimetrePerSecond
%%	\item hasDurationInMinutes
%%	\item hasFeedRateInKilogramPerHour
%%	\item hasFinishTimeValue
%%	\item hasStartTimeValue
%%\end{itemize}
%%
%%
%%
%%\subsubsection{SAREF}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item FeatureOfInterest
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item makesMeasurement ($\equiv$ measures)
%%	\item measurementMadeBy ($\equiv$ isMeasuredBy)
%%\end{itemize}
%%
%%
%%\subsubsection{SSN/SOSA}
%%
%%\begin{itemize}
%%	\item Property ($\equiv$ Characteristic)
%%	\item ObservableProperty
%%	\item Sensor
%%	\item Platform
%%	\item Stimulus
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item detects
%%	\item hosts
%%	\item isHostedBy
%%	\item observes
%%	\item isObservedBy
%%\end{itemize}
%%
%%
%%
%%\subsubsection{GeoSPARQL}
%%
%%\paragraph{Concepts}
%%
%%\begin{itemize}
%%	\item SpatialObject ($\equiv$ PhysicalObject)
%%	\item Feature
%%	\item Geometry
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasDefaultGeometry
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasMetricArea
%%	\item hasMetricLength
%%	\item hasMetricPerimeterLength
%%	\item hasMetricSize
%%	\item hasMetricVolume
%%\end{itemize}
%%
%%
%%
%%
%%\subsubsection{OM Ontology}
%%
%%\paragraph{Classes}
%%
%%\begin{itemize}
%%	\item Measure
%%	\item Unit
%%	\item hasUnit
%%\end{itemize}
%%
%%
%%\paragraph{Data Properties}
%%
%%\begin{itemize}
%%	\item hasNumericalValue
%%\end{itemize}
%%
%%
%%
%%\subsection{Our Signature}
%%
%%
%%\paragraph{Classes}
%%
%%\begin{itemize}
%%	\item DefectCharacteristic
%%	\item DefectSource ($+$ subclasses)
%%	\item Defect ($+$ subclasses)
%%	\item MetrologicalCharacteristic (find substitute?)
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
%%
%%\begin{itemize}
%%	\item hasMeasure (change? remove? find OM substitute?)
%%	\item isMeasureOf (change? remove? find OM substitute?)
%%	\item measures (find SOSA substitute?)
%%	\item isMeasuredBy (find SOSA substitute?)
%%	\item hasSource ($+$ subproperties)
%%	\item isSourceOf
%%\end{itemize}
%%
%%
%%\paragraph{Properties}
